Diffusion-ES: Gradient-free Planning with Diffusion for Autonomous Driving and Zero-Shot Instruction Following

Diffusion models excel at modeling complex and multimodal trajectory distributions for decision-making and control. Reward-gradient guided denoising has been recently proposed to generate trajectories that maximize both a differentiable reward function and the likelihood under the data distribution captured by a diffusion model. Reward-gradient guided denoising requires a differentiable reward function fitted to both clean and noised samples, limiting its applicability as a general trajectory optimizer. In this paper, we propose DiffusionES, a method that combines gradient-free optimization with trajectory denoising to optimize black-box non-differentiable objectives while staying in the data manifold. Diffusion-ES samples trajectories during evolutionary search from a diffusion model and scores them using a black-box reward function. It mutates high-scoring trajectories using a truncated diffusion process that applies a small number of noising and denoising steps, allowing for much more efficient exploration of the solution space. We show that DiffusionES achieves state-of-the-art performance on nuPlan, an established closed-loop planning benchmark for autonomous driving. Diffusion-ES outperforms existing sampling-based planners, reactive deterministic or diffusion-based policies, and reward-gradient guidance. Additionally, we show that unlike prior guidance methods, our method can optimize non-differentiable language-shaped reward functions generated by few-shot LLM prompting. When guided by a human teacher that issues instructions to follow, our method can generate novel, highly complex behaviors, such as aggressive lane weaving, which are not present in the training data. This allows us to solve the hardest nuPlan scenarios which are beyond the capabilities of existing trajectory optimization methods and driving policies.

==> OLD1_abstract.tex <==
\begin{abstract} 
%
Evolutionary  search methods such as Cross Entropy Method (CEM) and Path Integral (MPII)  optimize  black-box cost functions by  iteratively sampling and scoring trajectory proposals.  % and are ubiquitous in robot trajectory planning. 
They are ubiquitous in trajectory optimization thanks to their generality, but  %suffer from the curse of dimensionality because  often they %do not benefit from trajectory samples to learn sampling from the data manifold and 
%model cannot efficiently sample trajectories from the data trajectory manifold and 
%as a result 
 often waste compute sampling and scoring  unnatural, infeasible or uncommon trajectories. % since they do not model nor they can efficiently  sample  from the  trajectory data manifold. 
 %trajectory samples lying far from the data  manifold as they do . 
 Reward-guided trajectory diffusion  generates trajectories that  belong to a trajectory manifold, captured by a diffusion model, and maximize a differentiable reward function, by alternating between diffusion denoising steps and reward gradient steps with respect to the noised trajectory. The reward function has to be differentiable and is fitted to both clean and noised samples, which limits its applicability as a general trajectory optimizer. In this paper, we marry evolutionary  search  with  generative modelling  for trajectory optimization. We propose \model{}, a method
 %that marries evolutionary search and trajectory diffusion bringing the best of both worlds. \model{} 
 that can optimize arbitrary non-differentiable black-box objectives without reward function retraining by sampling  trajectory proposals using a truncated reverse diffusion process. 
 %from a trajectory diffusion model that captures a set of gives trajectory data. 
 The trajectory  mutation process  uses only a small number of noising and denoising steps, which renders \model{}  time efficient.
 It significantly accelerates optimization by focusing computation on  samples from the trajectory data manifold.  %which makes is computationally competitive to the original ES methods.
 We test \model{} in driving and language instruction following in nuPlan, an established benchmark for autonomous driving. We show it 
 %. We show it generates safe and compliant driving behaviors and 
 outperforms  sampling-based planners, reward-guided trajectory  denoising, as well as reactive diffusion-based and deterministic driving policy transformers.  
 For instruction following, we  automatically  map language instructions to programs  through few-shot LLM prompting, that shape the reward function optimized by \model{} and baselines. %, and control behaviour of the driving agent. 
%We validate our results in nuPlan and show that our approach can generate safe and compliant driving behaviors on a suite of challenging planning tasks. 
We show \model{} effectively optimizes  the generated reward functions %generated by natural language instructions through few-shot LLM prompting 
and infers highly complex behaviors, such as aggressive lane weaving,   not present in the training data, that  
%. Finally, we show that our planner can be used to 
solve the hardest nuPlan scenarios, while other planners or reactive driving policies fail to do so.
%trajectory sampling that combines the best of evolu
%They do not improve with more data and ths
%In this paper, we use diffusion models to perform language-guided closed-loop planning for autonomous driving. Conventional wisdom suggests one can use scene-conditioned diffusion policies with classifier guidance to flexibly plan over novel objectives at test-time. We show that excessive conditioning information can hinder downstream planning performance due to poor generalization and lack of diversity. Additionally, we show that gradient-based optimization (e.g. classifier guidance) can actually perform worse than sampling-based optimization (e.g. CEM/ES) for guided diffusion sampling at lower dimensionality, which we show experimentally. To that end, we demonstrate how a diffusion model with no conditioning information at all can be used to accelerate planning using online sampling-based guidance. We introduce a novel sampling-based guidance method DiffusionES which handles arbitrary non-differentiable black-box objectives without retraining. DiffusionES uses a truncated reverse diffusion process to denoise candidates which significantly accelerates optimization. We use LLMs to map language instructions to programs which adaptively control the behavior of our planner through reward shaping. We validate our results in nuPlan and show that our approach can generate safe and compliant driving behaviors on a suite of challenging planning tasks. Additionally, with language supervision our approach can synthesize highly complex behaviors (such as aggressive lane weaving) which are not present in the training data. Finally, we show that our approach can be used to solve the hardest nuPlan scenarios through language feedback from a human expert.
% We marry diffusion-based  generative models with zero-shot instruction-to-program generation with  Large Language Models (LLMs). We propose   a diffusion-based driving policy    that conditions on a tokenized  representation of the dynamic visual scene  and, optionally, a language instruction, and predicts a distribution over driving trajectories that follow traffic rules as well as the language instruction, when possible.  
% %for predicting a distrubution over car wayp
% %We propose a scene-conditioned trajectory diffusion policy, we call \model{}, for autonomous driving that  conditions on a tokenized scene representation of the dynamic visual scene, a far destination goal,  and, optionally, a language command, and predicts a driving trajectory that drives to the goal destination, following the language instruction if possible. 
% The model is trained from driving demonstrations to denoise noised vehicle trajectories, by attending to the scene context and a desired far destination goal. Our policy outperforms in driving ability its deterministic counterparts, as well as alternative trajectory generative policy formulations in the established nuPlan driving benchmark. 
% We show our policy can be controlled using natural language at inference time  zero-shot, without any additional training. Specifically, we prompt LLMs to map   language driving instructions to programs that output sets of waypoints on the road for the vehicle to reach or avoid. Inference in our diffusion policy using classifier-free guidance according to the program waypoint predictions 
% %We show  follows instruction in natural language by prompting Pretrained Large Language models to map language instructions to  programs that predict lanes and waypoints in the road for the vehicle to follow or avoid. 
% %The 
% controls the vehicle to change lanes, park behind another car,  change speed, keep distance from described landmarks, and combination of the above.   Handling multimodality in imitation learning for driving and following natural language  instructions are jointly handled in our diffusion-based formulation, thanks to the composability of diffusion generative models with additional constraints at inference time and their improved performance as  faithful generative models for modelling complex distributions. 

\end{abstract}



==> OLD2_intro.tex <==

\section{Introduction}

\topic{what is trajectory optimization and how it is done with evolutionary search and what are the pitfalls}
Trajectory optimization searches for an action trajectory that minimizes a cost function subject to dynamics constraints, and it is a parsimonious procedure in reinforcement learning and control \cite{}. In the case of general dynamics models, such optimization cannot be obtained with a closed form solution, and it is often addressed with variants of evolutionary search, such as, the cross entropy method (CEM) \cite{} or Path Integral Control (MPII) \cite{}. These  methods    sample action trajectory proposals,  score them using the designated cost function, and  sample new proposals in the vicinity of highest scoring ones (mutating the  elite samples). Evolutionary algorithms do not require the cost function to be differentiable, which  makes them general solvers across a wide variety of problem domains \cite{}.
 Albeit their generality and excellent performance in low dimensions \cite{}, they suffer from the curse of dimensionality because % often they %do not benefit from trajectory samples to learn sampling from the data manifold and 
 they neither model nor they can efficiently sample  from the  trajectory data manifold.  
%However, the process of sampling and mutating action trajectories is often quite naive and does not have general satisfying ways of sampling and mutating trajectories that being in the data trajectory manifold. 
Hand designed constraints on the way samples are generated are often employed, but they are not general enough to capture the idiosyncrasies of data samples,  they  are tailored to a specific task, and are hard to transfer across tasks. As a result,  evolutionary search methods  often waste  computation in sampling and scoring unnatural, infeasible or uncommon action trajectories, which hinders their performance. %rendering the search suboptimal or ineffective.

%; as a result, they  
%as a result 
% often waste compute on  unnatural, infeasible or uncommon samples.
\begin{figure}[t!]
  \centering
    \includegraphics[width=0.6\linewidth]{figures/approach_new.jpg}
  \caption{Closed-loop trajectory optimization with \model{} for driving and instruction following. \todo{here we need to put some impressive results from the model, and maybe comparison with vanilla CEM. They can driving results or language instruction following results.}}
  \label{fig:architecture}
\end{figure}

\topic{diffuser- guided trajectory sampling for trajectory optimization}
Diffusion models have recently been shown to excel at modeling highly complex and multimodal trajectory distributions for decision-making and control \cite{janner2022planning, Ajay2022IsCG}..
Recent approaches of blablabkla \cite{} and others  optimize trajectories under a differentiable reward function by alternating between denoising diffusion steps and backpropagating reward gradients to the noised trajectory. In this way, sampled trajectories are pushed towards the trajectory data manifold  while also maximizing the reward function at hand \cite{}. This decoupling of the reward function  and the trajectory diffusion permits the same trajectory diffusion  model to be used for maximizing a variety of learnt reward functions at test time. 
%This also has the added benefit of flexibility at test-time. 
However, it does require the reward function to be differentiable and fitted in both noisy and clean trajectories, which usually requires re-training. 
Alternatively, other methods train conditional diffusion trajectory prediction models through imitation learning from demonstrations \cite{},  %conditioning objectives during training, 
using rewards as conditioning information to the trajectory diffusion model \cite{DecisionDiffuser]} or finetuning the diffusion policy with reinforcement learning \cite{RL diffusion papers}. While these methods can handle black-box environment reward functions or demonstrations to imitate, using them off-the-shelf or with guidance under reward functions at test time fails when found out-of-the training distribution.   
%also require conditioning objectives to be available at training time and 
%struggle to generalize at test time \cite{}.  %$(?).
 Indeed, we show that excessive conditioning information can hinder downstream planning performance due to poor generalization and lack of diversity in the trajectory proposals. Our findings agree with recent work on energy based models where conditioning on the environmental context through additional constraints can better generalize over training an environment conditional diffusion model \cite{}. %composition at test time 

%Prior policies often guide the action sampling to accelerate such search \cite{}. 
%Recent advances of generative modelling and specifically diffusion models, have been used to model action trajectories, and are currently the most high fidelity samplers fromt he data manifold. They are trained to add varying amount of noise and remove it from datapoints. They sample from the data manifold by sampling white noise and then iteratively denoise it. %By learning to remove added noise to trajectory data samples, they learn to sample from the trajectory manifold through sampling white noise and then iteratively denoise it.
%and learning the data trajectory manifold. 
%Recent works have proposed to re-interpret trajectory optimization from the lens of generative modelling, and 
%by learning to sample from a trajectory manifold using trajectory diffusion model, and 
%optimize trajectories under a (differentiable) reward function by alternating between denoising generation steps and backpropagating reward gradients to the input action sequences \cite{}. In this way, the sampled trajectories are expected to both be on the data manifold and maximize the reward function. The reward function is trained on both noised sampled and clean samples since it is applied to both during sampling guidance.
%However, the need for differentiable reward functions makes guided trajectory sampling more restrictive in comparison  to black-box evolutionary algorithms that do not need reward functions to be differentiable. Also, the guided sampling at test time is unclear how effective it is into generating reward maximizing trajectories. 




%\topic{what we propose}
%\todo{MENTION: naive application would be prohibitely expensive: diffusion is already expensive and ES is very expensive}
In this paper, we ask the question: Can we combine the best of both worlds, generative diffusion trajectory modelling to sample and mutate samples from the trajectory manifold, and flexible black-box reward maximization of evolutionary search algorithms, for  general, faster and more effective trajectory optimization? We propose Generative Diffusion Evolutionary Search (\model{}), a method for trajectory optimization under general black-box objectives, not necessarily differentiable, that  learns a  trajectory diffusion model and uses it to sample and mutate trajectories during evolutionary search.  Naively combining sampling-based optimization with trajectory sampling from diffusion models does not work: Evolutionary algorithms like CEM or CMA-ES typically require many iterations to converge to good solutions, which, when combined with the computational cost of denoising inference, result in a prohibitively slow search process. 
%is highly nntrivial. Evolutionary algorithms like CEM or CMA-ES typically require many iterations to converge to good solutions, which, when combined with the computational cost of denoising inference,  leads to extremely slow search. 
%Additionally, since these optimizers treat their objective functions as black boxes, the process of sampling and mutating trajectories is highly inefficient and does not exploit prior knowledge from our model. 
%Ideally sampled trajectories should be constrained to the data manifold to avoid wasting computation on unfeasible trajectories.
In \model{}, trajectories are mutated using a \textbf{truncated  noising process},  by adding a small amount of noise to high scoring trajectory samples, and denoising them back. The amount of added noise is progressively decreased across search iterations. This renders \model{} computationally viable. The trajectory diffusion model can be optionally conditioned on any  scene information to allow sampling of scene-relevant trajectories. Interestingly, we found that such  conditioning information  narrows the trajectory distribution that trajectory proposals are sampled from, and hinders performance of \model{}. 

We test \model{} in its ability to infer driving trajectories in NuPlan \cite{}, an established driving benchmark that uses estimated ground-truth perception of vehicles, road lanes and traffic signs and their state for decision making. 
We empirically show the \model{} generates safe and compliant driving behaviors on a suite of challenging planning tasks. We show it outperforms  existing evolutionary search methods, such as CEM and MPII, reward-guided diffusion trajectory sampling (when this is applicable, i.e., for differentiable objectives), reactive neural transformer policies that directly map the surrounding traffic state  to ego-vehicle trajectories, using diffusion or deterministic models. 
%currently used  for trajectory optimization, performs equally well to hand-tailors planners that engineer the trajectory proposals \cite{},  as well as guided diffusion trajectory sampling, as well as reactive neural transformer policies that reactively map the surrounding traffic state  to road trajectories, using diffusion or deterministic models. 
We further test our model in its ability to infer trajectories that follow natural language driving instructions. We use Large Language Models (LLMs) to map language driving instructions to programs that \textit{shape} the driving reward function to  optimize by \model{}, by removing  vehicle actors that need to be ignored, added for vehicles that need to be paid attention to or yielded to, adding go-to sets of waypoints for following or changing lanes, speed constraints for accelerating or slowing down. \todo{details on what exactly these programs do}. %, which in turn  control the behavior of our planner through through reward shaping. 
%We validate our results in nuPlan and show that our approach can generate safe and compliant driving behaviors on a suite of challenging planning tasks. 
\model{} effectively optimizes  the LLM-generated reward functions % with language supervision our approach can 
and generates  highly complex behaviors, such as aggressive lane weaving or \todo{++}, which are not present in the training data. Last,  closed-loop planning with \model{} using sparse language instructions from a human expert %and corresponding adaptation of the reward function based on the environment's states, 
can solve the hardest nuPlan scenarios, making our model akin to a new driver that uses guidance from a human teacher for deciding when to yield, pass or merge in lanes. 



% through language feedback from a human expert. 





In summary, our contributions are as follows:
\begin{enumerate}
\item We introduce \model{} a trajectory optimization method that  can maximize general black-box objectives by learning  a trajectory sampler  with a diffusion model. It mutates elite trajectory samples using a truncated denoising process. To the best of our knowledge this is the first work to combine evolutionary search with generative models. %We mutate elite samples through a truncate denoising proc
%The first diffusion-based driving policy, with SOTA performance in an established driving simulation benchmark.
\item We conduct numerous experiments and comparisons against evolutionary search methods, reactive neural trajectory transformers (diffusion-based or deterministic), and NuPlan-tailored planners \cite{} and we show our method  outperforms the former and matches the performance of the later, generating much more diverse and flexible behaviours.
%Language controllability of a diffusion-based policy zero shot, without any instruction-trajectory training pairs, based on LLM instruction-to-program generation.
\item We showed \model{} can be used for optimizing black-box reward functions generated from natural language driving instructions through few-shot LLM prompting. No other optimizer was able to  effectively optimize the complex generated reward functions, which were a combination of the NuPlan environment rewards and shaping from  language instructions. 
\item We provided  an existential proof that NuPlan driving benchmark can be solved to 100\% accuracy if a human teacher is sitting next to an autonomous vehicle, and directing it in natural language with \model{} inferring trajectories that optimized the language-shape reward functions, minus the slowness of the planning.  % and directing a neural planner 
\item Through extensive comparisons we show the trade-off between conditioning information in neural models and their generalization through unconditional sampling and composition at test time with various reward functions, agreeing with results  in the manipulation literature  \cite{}.
\end{enumerate}
We believe \model{} is a general optimizer with applicability beyond driving. Our code and models will be publicly available upon publication. 



==> OLD_related.tex <==
\section{Related work}
\todo{to cite VoxPoser}


\paragraph{Learning versus Planning for Autonomous Driving}
\todo{talk here also about traj. optimization}
\todo{a lot of things can be copy pasted by the ldm planner paper related work}
%\paragraph{Learning to drive with imitation learning}
Pomerleau \cite{alvinn} first showed in 1989 how  a shallow neural network
 could be trained  from  driving demonstrations  to follow the road using  camera and laser range data as input using behaviour cloning. 
 To handle drifting, recovery situations were synthesized with a simulator, in the form of  side road images paired with  steering actions that would push the vehicle back in the  center of the road.   
%Decades-old work on ALVINN (Pomerleau (1989)) showed how a shallow neural network
%could follow the road by directly consuming camera and laser range data. 
  %Kinesthetic imitation learning for driving is particularly convenient as the actions of the human driver can be easily logged. 
Learning to drive from demonstrations 
in an end-to-end manner has seen a resurgence in recent years \cite{DBLP:journals/corr/abs-1710-02410,endtoendNVIDIA,gaildriving}. 
    Imitation learning methods  train neural network policies to map input to car waypoint trajectories \cite{endtoendNVIDIA}. 
Sensor-based  methods take as input images and, optionally,  LiDAR sensor readings \cite{neat,LBC,LAV},  while state-based methods take as input oracle perceptual representations represented as rasterized BEV maps of lane, vehicle and traffic sign information \cite{chauffernet,roach},  %perspective semantic segmentation maps \cite{modularity},
or as scene token graphs 
%as input to graph neural networks or transformer networks
\cite{plant}; our model belongs to this last category. Driving benchmarks exist for both sensor-based and state-based methods. For example, the CARLA benchmark \cite{CARLA} is focused on learning to drive from sensory input, while NuPlan, which we use, focuses on driving from tokenized scene representations \cite{caesar2022nuplan}. Methods that drive from pixels address the problem in its total complexity but  confound  perceptual mistakes with behavioural mistakes:   it is not easy to attribute driving failures to perceptual mistakes or to behavioural ones, due to the black box nature of neural networks. On the contrary, state-based  methods isolate perception from behaviour and demonstrate what can be achieved with oracle perception, and what behavioural mistakes still need to be addressed. 




%Recent work by Chen et al. (2015) demonstrated a convolutional net to estimate affordances such as distance to the preceding car that could be used to program a controller to control the car on the highway.
%Bojarski et al. \cite{endtoendNVIDIA} showed how to train a deep convolutional neural network from driving demonstrations to  steer a car by consuming camera input. 
%A three-camera rig was used to automatically generate augmentation data, in the form of images paired with recovering steering actions from the left and right cameras. 
%Kuefler et al. \cite{gaildriving} use Generative Adversarial Imitation Learning (GAIL) as an alternative to augmentations to overcome cascading errors typically present in behavior cloned policies  so that they are more robust to perturbations. 
%Codevilla et al. \cite{DBLP:journals/corr/abs-1710-02410}  train a network using camera inputs and conditioned on high-level commands to output steering and acceleration. 


%Some 



%Driving simulator environments and benchmarks, such as the CARLA simulator \cite{CARLA}, have enabled research on  neural driving policies trained and deployed in simulation, as well as  on sim2real transfer of driving policies. They further give the opportunity of using reinforcement learning, instead of imitation learning, to acquire driving behaviours \cite{roach,endtoendRL}. Neural driving policies in recent years developed within such simulation environments can be categorised in two main families:

One application domain that involves similar challenges
to driving is offline motion trajectory forecasting \cite{rulesroad,multipath,multimodal,DESIRE,trevorcar,R2P2,precog,wayformer, scenetransformer, autobots, stackedtransf, endtoendraquel}. While evaluating driving performance requires a simulator, evaluating offline trajectory performance only requires a datasets of driving trajectories. There are multiple such datasets, such as, Argoverse \cite{Argoverse}, Waymo Open Dataset \cite{Sun_2020_CVPR}, and nuScenes \cite{nuscenes}, to name a few.
% \todo{BRIAN what are other datasets?}. 
%Imitation learning for offline trajectory prediction or closed-loop control suffers from multimodality of expert trajectories. Regressing car waypoints assumes that a car waypoint follows a unimodal Gaussian distribution in the 2D BEV space. 
%Building upon progress in generative models, motion trajectory decoders have been proposed that can model multimodal trajectory distributions.
Many methods attempt to predict a distribution over future trajectories instead of a single trajectory, for the ego-vehicle or coordinated among multiple agents in the scene.  Tang and Salakhutdinov use conditional variational autoencoders (CVAEs) with discrete latent variables  \cite{multiplefutures}, Rhinehart \etal \cite{R2P2} use symmetric cross-entropy losses between predicted and ground-truth trajectory distributions,  Ngiam \etal \cite{scenetransformer} use multiple prediction heads with join classification and regression losses, Girgis \etal use set latent  variables \cite{autobots}. %, Zhong \etal use  diffusion models \cite{controllabletraffic}. 


Learning to drive from imitating  driving demonstrations is prevalent in the research and development of autonomous vehicles \cite{DBLP:journals/corr/abs-1710-02410,endtoendNVIDIA,gaildriving}.  %All methods 
Driving policies can take as input pixel and LiDAR input \cite{alvinn,endtoendNVIDIA,LBC,LAV,transfuser}, or use ground-truth perception of lanes, vehicles,  traffic signs and their  state attributes \cite{chauffernet,plant,roach}. In both cases, most methods predict  waypoints for the vehicle to follow, conditioned on a scene and a  distant goal representation. %Though learning from demonstrations is an established learning method, 
Most imitation learning methods optimize an objective that boils down to cloning the actions of the expert, as proposed  by Pomerleau decades ago \cite{alvinn}. Behaviour cloning has an underlying assumption of a unimodal Gaussian distribution for the actions to predict, which cannot handle  multimodality of  experts' driving behaviours, especially prevalent during accelerations, lane changes, merges, etc. . % Indeed, some many drive faster or slower, merge or bypass a car. %, and such multimodality cannot be adequately modelled by a unimodal Gaussian distribution.   
%hurts action regression, which is essentially what almost all methods have been using. 
%The limitations of behaviour cloning in the presence of multimodal action distributions is well documented in the literature \cite{}. 
Objectives and architectures that can better handle multimodal trajectory prediction have been  proposed,  
such as, mixture of expert  trajectory decoders \cite{wayformer}, combining classification and regression losses \cite{shafiullah2022behavior}, using Gaussian trajectory mixtures \cite{Kim_2023},   
conditional variational autoencoders (VAEs) with continuous or discrete latent variables \cite{multiplefutures, fragkiadaki2017motion}, producing heatmaps over a 2D bird's-eye-view  map to sample waypoint trajectories from \cite{lookout}. 

% such as, conditional VAEs with continuous or discete latent variables \cite{}, Gaussian mixture models \cite{}, or having multiple heads that are scored \cite{},  combination of regression and classification losses \cite{}.
 
%Most have been tried for offline traj. prediction and not for closed loop control. We compare with behaviour transformer in our experimental section.





%either drive from pixel and LiDAR input\cite{alvinn,endtoendNVIDIA,LBC,LAV,transfuser}, or use ground-truth perception of lanes, vehicles,  traffic signs and their  state attributes \cite{chauffernet,plant,roach}. The former set of methods build  neural architectures that lift 2D perspective camera features to stable 3D feature maps, or directly fuse perspective feature to predict  future waypoint trajectories; 
%their performance on the CARLA leaderboard \cite{CARLA}, a popular driving simulation environment, is impressive and the driving performance has been steadily increasing over the years. 
%This set of methods
%Driving from pixels compounds mistakes of perception and driving behaviour.  The latter set of methods isolate mistakes of perception and driving behaviour and are motivated by the large-scale annotation efforts of the self-driving vehicle industry to annotate oriented 3d boxes of vehicles,  bikers, pedestrians and traffic sings, as well as the use of high definition maps.  Surprisingly, few models have been developed for the latter case; though numerous methods exist for offline vehicle motion trajectory forecasting from oracle overhead rasterized maps or scene graphs \cite{wayformer, scenetransformer, autobots}, very few attempt to drive using this representation. %As a result, it is often hard to know how muc



%\paragraph{Diffusion models for robot control} Diffusion models have recently brought a revolution in generative modeling by being able to faithfully capture the distribution at hand, without dropping modes and without hallucinating ones, in multi domains, such as text-to-image generation \cite{saharia2022photorealistic}, image-to-image translation \cite{saharia2022palette}, view synthesis \cite{watson2022novel}, 3D point cloud generation \cite{nichol2022pointe}, and many others. %images conditioned on text or other images \cite{}.   The problem of multimodality in imitation learning is not only for driving but for any control domains, such as , manipulation.   Work of \cite{chi2023diffusion,pearce2023imitating}  showed that diffusion models can predict robot actions for imitating expert manipulation trajectories and better handle multimodality in imitation that previous alternative formulations. 

\paragraph{Generative models for robot control} Diffusion models \cite{SohlDickstein2015DeepUL,ho2020denoising,song2020denoising,nichol2021improved} learn to approximate the data distribution through an iterative denoising process, and have shown impressive results on both unconditional and conditional image generation \cite{Dhariwal2021DiffusionMB,Saharia2022PhotorealisticTD,Rombach2021HighResolutionIS,Ramesh2022HierarchicalTI}. 
Diffusion models have been used in imitation learning for learning manipulation tasks \cite{chi2023diffusion,pearce2023imitating}, for controllable vehicle motion generation \cite{Zhong2022GuidedCD,Jiang_2023_CVPR} and for video generation of manipulation tasks \cite{Du2023LearningUP}.  
%In the field of robotics, diffusion models find applications on planning \cite{janner2022planning,Ajay2022IsCG,Huang2023DiffusionbasedGO}, %scene re-arrangement \cite{Kapelyukh2022DALLEBotIW,Liu2022StructDiffusionOD}, 
%controllable motion optimization \cite{Zhong2022GuidedCD,Jiang_2023_CVPR}, and imitation learning \cite{chi2023diffusion,reuss2023goal}. 
Their main advantage is that they can better capture the action trajectory distribution compared to previous  generative models. In this work,  we explore their performance in learning to drive from demonstrations, as well as their controlability from language instructions. 
%are that i) they are multimodal and stable to train \cite{chi2023diffusion}, thus being able to absorb raw non-expert data without collapsing to a single suboptimal behavior, ii) they better capture the full distribution compared to other generative model alternatives \cite{urain2022se}. 
%Recent works use diffusion model to predict complete trajectories, often auto-regressively \cite{chi2023diffusion,pearce2023imitating}.   
% As our experiments demonstrate, such a design choice struggles with long-horizon tasks, especially in a multi-task setting. 
%Instead, we use diffusion models to generate local trajectories that are chained together with macro-actions. %smooth and physically-plausible local trajectories.



\paragraph{LLMs for zero-shot semantic parsing and  instruction following}
LLMs trained from Internet-scale text have shown impressive zero-shot reasoning capabilities for a variety of downstream language tasks \cite{brown2020language} when prompted appropriately, without any weight fine-tuning \cite{DBLP:journals/corr/abs-2201-11903,DBLP:journals/corr/abs-2107-13586,brown2020language}. 
%Large language models (LLMs)  are trained with Internet-scale text to autoregressively predict the next word conditioned on prior text context using billions of parameters. At this scale of parameters and training data, an interesting phenomenon of in-context learning emerges \cite{brown2020language}, where at test time, the LLM is directed to complete new tasks it was not trained on  with appropriate text pre-conditioning, which is called a prompt \cite{liu2021pretrain}. %Zero shot and few shot prompting are used to elicit analogous responses to question - answers pairs as the prompts \cite{DBLP:journals/corr/abs-2107-13586}. 
%Work of code-as-policies \cite{} and its subsequent descendants showed how LLMs can map manipulation instructions, such as `` " to programs that call ready  low-level short-term policies or skill controllers  with appropriate plan-like prompts \cite{https://doi.org/10.48550/arxiv.2204.01691,singh2022progprompt,liang2022code}. Works of    
 LLMs have been shown to map instructions to language subgoals \cite{DBLP:journals/corr/abs-2012-07277,DBLP:journals/corr/abs-1909-13072,huang2022language,https://doi.org/10.48550/arxiv.2207.05608} or python programs \cite{liang2022code,surís2023vipergpt,Gupta_2023_CVPR,hsu2023ns3d} with appropriate plan-like prompts. The predicted  programs or subgoals  interface with  low-level short-term policies or skill controllers \cite{https://doi.org/10.48550/arxiv.2204.01691,singh2022progprompt,liang2022code} or pretrained vision-language detectors \cite{surís2023vipergpt,Gupta_2023_CVPR,hsu2023ns3d}.  
%LLMs trained from Internet-scale text have shown impressive zero-shot reasoning capabilities for a variety of downstream language tasks \cite{https://doi.org/10.48550/arxiv.2005.14165} when prompted appropriately, without any weight fine-tuning \cite{DBLP:journals/corr/abs-2201-11903,DBLP:journals/corr/abs-2107-13586}.  
The scene description is usually provided in a symbolic form as a list of objects present, predicted by open-vocabulary detectors \cite{DBLP:journals/corr/abs-2104-12763}. 
Works of \cite{liang2022code,https://doi.org/10.48550/arxiv.2209.00465}  also feed as input overhead BEV spatial coordinates of objects to inform the LLM's predictions. 
%ViperGPT \cite{surís2023vipergpt} and visual programming \cite{Gupta_2023_CVPR}  and \cite{hsu2023ns3d}  map questions and referential expressions to programs over visual-language pre-trained models for object detection and grounding \cite{zeng2022multigrained, zhang2022glipv2,li2023blip2}. They show such programmatic decomposition helps out of distribution in comparison to end-to-end attention based question answering and referential grounding. 
Our work is most related to code-as-policies \cite{liang2022code} and extends it to the driving domain and language instructions there in. Instead of interfacing with ready low level pick and place manipulation controllers as \cite{liang2022code}, we use the set of waypoints and corresponding cost maps predicted by the programs to  control a  diffusion-based driving policy. 



Parallely, controlling an autonomous vehicle in natural language will  enable  human passengers to influence the vehicle's route and behaviour beyond supplying a final goal destination. Passengers would be able to give feedback to the vehicle and suggest places to park, intermediate stops, vehicles to follow, lanes to prefer or change, or speed to use. Language controllability of an autonomous vehicle is important for versatility and personalization of the vehicle-human experience,  and for reinforcing trust and transparency  in human-vehicle interaction. 

Our language controllability builds upon code-as-policies \cite{liang2022code} in that it  prompts LLMs to predict programs for parsing instructions. Instead of predicting coordinate locations for pick and place control primitives which directly  parametrize the robot actions, our model combines predicted waypoints with a trajectory diffusion model to predict actions that both comply with a trajectory prior and attempt to follow the instruction. In that sense, we do not expect the LLM to know how to drive; this is the responsibility of the driving diffusion model. The LLM is merely responsible for interpreting language as cost maps to guide trajectory diffusion sampling. For example, the instruction \textit{``merge in the left lane"} should predict a program that outputs low cost for all waypoints in the left lane; the one most suitable to reach based on the current velocity and scene context should be selected during guided trajectory diffusion sampling.
%LLMs were used to generate task curricula and predict skills to execute in Minecraft worlds \cite{zhu2023ghost,lifshitz2023steve1}. Methods of \cite{wang2023voyager} use privileged information from the Minecraft simulator's interface regarding failures, state and inventory which they use to feedback to an LLM to plan and re-plan based on sub-goal successes and failures. LLMs are used as knowledge bases in place of traditional tuple based knowledge  \cite{roberts2020knowledge,brown2020language}. 


Closest to our work are the recent method of \cite{controllabletraffic} and concurrent work of \cite{MotionDiffuser}. %While these methods 
%\todo{DETAILS:
They both show that diffusion models can be used for forecasting offline vehicle trajectories, and controlling  them via attracting them or repelling them from specific waypoints, or using cost maps related to traffic rules. % using classifier free guidance.} 
The methods are motivated by controllability of diffusion models at inference time. 
%Work of \cite{MotionDiffuser} further evaluates offline trajectory performance using minSADE, a top-6 trajectory matching metric, and shows state-of-the-art performance. 
%The proposed models do not outperform the previous work in offline trajectry prediction in the 
%None compares on estblished benchmarks  and not by improved offline trajectory performance. 
Our work is inspired by these works; instead of offline trajectory prediction it is the first to use diffusion policies for closed-loop driving and outperform previous formulations in nuPlan. %While in top-1 offline trajectory prediction error our method is worse than the baselines, it is able to better captures the trajectory distribution in rare  scenarios such as turns, leading in improved online driving performance. 
%Our experiments show that this is significant: the offline performance of diffusion policy was worse than existing deterministic alternatives. However, in rare scenarios critical for driving, diffusion better captures the trajectory distribution, leading in improved driving performance. 
Furthermore, we are the first to show language controllability of diffusion policies by marrying diffusion with LLM prompting for instruction-to-program generation. %\todo{++}



==> OLDexperiments.tex <==
\section{Experiments}

We evaluate our approach on nuPlan \cite{caesar2022nuplan}, a large-scale planning benchmark for autonomous driving.

%First, we show that our approach outperforms several strong learning baselines on challenging closed-loop planning scenarios, highlighting the effectiveness of diffusion models for capturing multimodal human driving behaviors.
%Next, we evaluate our approach for language-guided planning, showing quantitatively that our controllability approach outperforms other state-of-the-art techniques for guided diffusion in trajectory prediction.
We also compare the performance of LLM planners to oracle baselines which have access to ground-truth goal waypoints.
Finally, we qualitatively demonstrate how our novel prompting approach enables us to generate composable closed-loop plans.

% OUTLINE
% nuPlan driving scores
% point reaching language task (just the in-distribution version for now). broken down into:
% a) controllability methods
% b) language vs GT
% qualitative stuff :D examples of programs

  %   \begin{figure*}[h!]
  %   \centering
  %     \includegraphics[width=0.95\linewidth]{figures/qualitative.png}
  %   \caption{\textbf{Qualitative driving results of our model} in the nuplan benchmark. Our model solves a variety of challenging driving scenarios including unprotected left turns (row 1), unprotected right turns (row 2), and lane changes (row 3). We also visualize some failure cases of our model. Our model can be susceptible to deadlocking at intersections due to over-conservative behavior (row 5). Additionally, our model struggles with lane changes (row 6). For driving video results, please see our supplementary file.
  %   }
  %   \label{fig:qualitative}
  % \end{figure*}

\begin{figure}[t!]
\centering
\begin{tabular}{c}
  \includegraphics[width=0.98\linewidth]{figures/diffusion_p1.png}\\
  \includegraphics[width=0.98\linewidth]{figures/diffusion_p2.png}
\end{tabular}
  \caption{\textbf{Output predictions for our diffusion-based driving policy.} The \color{cyan} cyan \color{black} trajectory is the ground-truth, the \color{purple} dark red \color{black}  trajectories are the trajectory samples, and the white trajectory is the highest likelihood sample. Likelihoods of trajectories are computed as described in \cite{MotionDiffuser}.}
\label{fig:qualitative}
\end{figure}

\subsection{Unguided Closed-Loop Planning}
We first consider the original nuPlan closed-loop planning task without language guidance.
nuPlan consists of three increasingly complex modes: open-loop planning, closed-loop planning with non-reactive agents, and closed-loop planning with reactive agents.
In this work, we are only concerned with closed-loop planning with reactive agents.
For this task, the benchmark assigns agents a composite metric score which consists of multiple components relating to driving performance (e.g. at-fault collisions, lane following, rider comfort, etc.). A more detailed breakdown of these metrics can be found on the nuPlan challenge website \cite{caesar2022nuplan}.

We compare to the following baselines:
\begin{itemize}
    \item \textit{Unimodal/deterministic imitation}: a simple behavior cloning agent that deterministically predicts a single action
    % \item \textit{Behavior Transformer \cite{shafiullah2022behavior}}: a state-of-the-art multimodal imitation agent which combines both action binning and continuous residual prediction
    \item \textit{IDM planner}: a manually-tuned planning agent which uses heuristics to avoid collisions and maintain comfortable distance from leading vehicles
\end{itemize}

For both learned baselines, we compare to our own re-implementations using the same encoder backbone as our proposed diffusion approach.
All models are trained on the same offline dataset of 2.5 million samples.

% \subsection{Driving performance}
\begin{table}
\begin{center}
\begin{tabular}{l|c}
\hline
Method & Score $\uparrow$ \\
\hline
Unimodal/deterministic & 63 \\
% Behavior Transformer & 46 \\
IDM planner & 71 \\
Ours & 69 \\
\hline
\end{tabular}
\end{center}
\caption{\textbf{Driving performance on nuPlan.}
%all perception-based and state-based methods that use the same distance subgoal direction representation.
}
\label{tab:longest6}
\end{table}

We report our results in Table \ref{tab:longest6}. Our diffusion-based approach outperforms both imitation learning baselines and achieves comparable driving score to the manually-tuned IDM planner.

\subsection{Language-Guided Planning}

Next we show how our approach can be re-tasked to perform language-conditioned planning without any additional training.
% \subsubsection{Goal reaching using language commands}
We perform a quantitative evaluation of our controllability approach for simple goal reaching tasks.
We evaluate on a selection of 10 scenarios from the nuPlan dataset.
For each scenario, we set the actual location of the ego vehicle after 8 seconds to be our ground-truth goal point.
Then, we manually generate a natural language command describing the behavior of the ego vehicle in the scenario.
The objective in each scenario is to reach the goal location given only access to natural language commands.

To the best of our knowledge, no prior works have explored language controllability specifically for driving.
Therefore, we compare to several ablations of our proposed approach.
First, we consider several alternative approaches to goal-conditioned and constrained diffusion sampling. \todo{++}
% Additionally, we also compare performance when using LLM-inferred waypoints to ground-truth waypoints to illustrate the effectiveness of the LLM planner at predicting goals from natural language.
% we compare our model against the following baselines:


 
% \begin{itemize}
% \item \textbf{Oracle Language Controllability}: Previous works, such as Motion-Diffusor \cite{}, assume access to attractor and repellor waypoints to guide the trajectory of diffusion models towards the goal. In our work, we aim to relax the reliance on oracle waypoints by https://www.overleaf.com/project/647a0f6d693c8af9000122cdusing language instructions to communicate the goals. However, in this baseline, we provide oracle goal waypoints to the diffusion policy as an upper bound for performance with language as the communication medium. This also enables us to quantify the performance loss when using language instructions.
%     \item \textbf{Brian: some other variant of our models}
% \end{itemize}
% \todo{BRIAN - AYUSH}

% \begin{figure*}[h!]
%     \centering
%     \includegraphics[width=.95\linewidth]{figures/test_qual2.pdf}
%     \caption{Caption}
%     \label{fig:enter-label}
% \end{figure*}

\begin{table}
\begin{center}
\begin{tabular}{l|l|c|c}
\hline
Goal Type & Constraint Method & Successes $\uparrow$ & Average Distance Error $\downarrow$ \\
\hline
Oracle & Ours & 10/10 & 0.0 \\
Oracle & MotionDiffuser \cite{MotionDiffuser} & 5/10 & 11.56 \\
Oracle & CTG \cite{controllabletraffic} & 6/10 & 3.30 \\
Oracle & In-painting & 6/10 & 6.11 \\
\hline
Natural language  & Ours &  6/10 & 6.04 \\
Natural language  & MotionDiffuser & 6/10 & 6.87 \\
Natural language  & CTG & 7/10 & 2.91 \\
Natural language  & In-painting & 6/10 & 7.01 \\
\hline
\end{tabular}
\end{center}
\caption{\textbf{Controllability results in nuPlan.}}
\label{tab:controllability}
\end{table}

\subsection{Limitations - Future directions}
%closed loop open loop
Our framework has currently the following limitations:
\textbf{1.} Inference speed. Our diffusion model operates at 0.5Hz, which is much slower than our non-diffusion baselines and too slow to run in real-time.
We envision a system that learns to switch between cheap waypoint regression in easy scenarios and a expensive diffusion-based waypoint prediction in more challenging scenarios.
\textbf{2.} It cannot handle instructions that need predictions of the behaviour of other agents, e.g., \textit{``yield to the incoming vehicle"}. 
Predicting multi-agent trajectories instead of only the ego vehicle's trajectory would allow to follow this type of instructions as well. 
\textbf{3.} Lack of large-scale  benchmark of language controllability for driving policies. Development of a large scale benchmark for vehicle-human interaction through language would help spark more research in this direction. All the above are exciting avenues for future work. 

%The encoder has access only to object motions and state attrbutes. There may be more important features to take into account when predicting agents' behavour 
%Application of 
%It has access to ground-truth perception. While for urban scenes access to this representations= is reasonable thanks to the large scale annotation effortds 
%As shown in Figure \ref{fig:qualitative}, our model struggles with multi-lane scenarios and gets stuck in 4-way intersections. Many of these scenarios are also challenging for our autopilot expert. Our model being an imitation learning model is upper bounded by the autopilot's performance.  Handling these scenarios using architectural innovations as well as combination of imitation and reinforcement learning  are direct avenues for future work. 
%that will help 
%In our fu
%Handling these cases, as well as, improving the driving score  

%\todo{In the following sections, we both quantitatively and qualitatively evaluate our model's ability to identify relevant actors. ?}

% \subsubsection{Quantative evaluation via RFDS}

% % figure 1: longest6 benchmark numbers
% \begin{table}
% \begin{center}
% \begin{tabular}{|l|c|}
% \hline
% Method & RFDS $\uparrow$ \\
% \hline\hline
% Inverse Distance \cite{plant} & 29.13 \\
% PlanT \cite{plant} & 96.82 \\
% \model{} (ours) & $\infty$ \\
% \hline
% \end{tabular}
% \end{center}
% \caption{\textbf{RFDS}. Each approach is evaluated by executing the rule-based autopilot while only passing in the most relevant actor according to the attention scores extracted from each method. Relative Filtered Driving Score is then calculated by taking the resultant driving score and }
% \label{tab:longest6}
% \end{table}

% Following \cite{plant}, we evaluate a variant of our method where we use the attention scores from our model to selectively filter the input to the rule-based autopilot used to collect our demonstration data.

% \subsubsection{Qualitative evaluation}






==> OLDmethod.tex <==

\begin{figure*}[h!]
  \centering
    \includegraphics[width=0.975\linewidth]{figures/approach_new.jpg}
  \caption{\textbf{Diagram for \model{}.} \textit{Top:} We show the sampled proposals across iterations for \model{} for the instruction ``". 
  %Staring from a set of proposals sampled from the trajectory diffusion model (shown in blue) we score each one and resample the top $k$ \%. 
  \textit{Bottom:} Mutation through truncated denoising. We show the trajectory resamples for different amount fo added and denoised noise, starting from the proposal at the leftmost column.
  %Resampling (a.k.a. mutation) happens through truncated noising and denoising process, where we add noise to the elite trajectories and denoise them (
  %Our model attends to a tokenized scene representations contextualized through a multi-layer transformer  and predicts the noise in a noised vehicle trajectory. At inference time, starting from Gaussian noise at each trajectories waypoints, iteratively denoises the trajectory to generate a sample from the scene condition vehicle trajectory distribution. Language instructions are mapped to programs that output waypoints for the car to reach of avoid. These are used as cost maps  during trajectory inference and guide vehicle trajectory prediction. %using classifier-free guidance.
  %\todo{MAKE FIGURE: we need to show the denoising of a trajectory, we need to show an instruction and the predicted program, then we need to show the denoising with waypoint constraints from language}
  }
  \label{fig:architecture}
\end{figure*}

\section{Method}  \label{sec:method}


The architecture of \model{} is shown in Figure \ref{fig:architecture}. 
%We consider the problem of ego-vehicle trajectory prediction conditioned on
%It is a generative model of driving trajectpries that 
It takes as input a tokenized representation of the input scene in terms of dynamic agents (cars, pedestrians, bikers), traffic lights  and road segments, as well as an optional natural language instruction  
%We learn a policy $\pi(\tau | s)$  that 
and predicts a fixed-length future trajectory $\tau$ for the ego-vehicle.
%given a state representation $s$.
We assume access to a dataset $\mathcal{D}=\{S_1, S_2, \dots, S_M\}$ of $M$ demonstrations, where $S_i$ contains annotations for the scene static map and accurate trajectories for all agents in the scene. %We model the distribution of all possible future trajectories with a diffusion model. 
We show that during inference we can jointly optimize for trajectory prediction and instruction following.
%using classifier-free guidance as well as programs generated by LLMs. 
%Figure \ref{fig:architecture} illustrates our full pipeline.
We describe the details of our diffusion-based policy in Section \ref{sec:policy} and its controllability from language instructions in Section \ref{sec:controlability}. %language-controllable trajectory generation in the following subsections.


\subsection{Diffusion driving policy} \label{sec:policy}

\paragraph{Diffusion-based trajectory generation} 
Let $\tau$ be a trajectory, predicted from a policy $\pi(\tau|s)$, with $s$ the state representation. We model  trajectory generation as a continuous diffusion process, which approximates the training distribution by sampling a noisy trajectory $\tau_0 \sim \mathcal{N}(0, \sigma_{max}^2\mathbf{I})$ and sequentially denoising it into trajectories $\tau_i$ with noise levels $\sigma_0 = \sigma_{max} > \sigma_1 > \dots > \sigma_N = 0$, so that at each noise level $\tau_i \sim p(\tau_i; s, \sigma_i)$. The endpoint $\tau_N$ of this process follows $p(\tau_N; s, \sigma_N) = \pi(\tau|s)$.

Following \cite{Song2020ScoreBasedGM,Karras2022ElucidatingTD}, we describe the diffusion process as a continuous-time differential equation:
\begin{equation}\label{eq:ode}
    d\tau = -\dot{\sigma}(t) \sigma(t) \nabla_\tau \log p\big(\tau; s, \sigma(t)\big)dt
\end{equation}
Note that $\sigma$ is a time-dependent variable with $\sigma_i = \sigma(t_i)$. We set $\sigma(t_i) = t_i$, following \cite{Karras2022ElucidatingTD}. The quantity $\nabla_\tau \log p(\tau; s, \sigma(t))$ is the \textit{score function} and indicates the direction towards higher density of training data under each noise level. It can be shown \cite{Karras2022ElucidatingTD} that the denoiser function $D_{\theta}$ that minimizes the expected denoising error for samples drawn from the training distribution for every noise level satisfies the equation:
\begin{equation}\label{eq:solution}
    \nabla_\tau \log p\big(\tau; s, \sigma(t)\big) = \frac{D_{\theta}\big(\tau; s, \sigma(t)\big) - \tau}{\sigma(t)^2}
\end{equation}
The denoiser function is implemented as a weighted sum of the input trajectory and the output of a neural network $F_{\theta}$:
\begin{equation}\label{eq:network}
    D_{\theta}\big(\tau; s, \sigma(t)\big) = c^{(t)}_{skip}\tau + c^{(t)}_{out}F_{\theta}(c^{(t)}_{in}\tau; s, c^{(t)}_{noise})
\end{equation}
where $c^{(t)}_{skip}, c^{(t)}_{out}, c^{(t)}_{in}, c^{(t)}_{noise}$ are scalar functions of $\sigma(t)$ (see Section \ref{sec:implem} for details).

During training, we sample noise $\epsilon \sim \mathcal{N}(P_{mean}, P_{std}^2\mathbf{I})$ \cite{Karras2022ElucidatingTD}, add it to a ground-truth trajectory $\tau_{gt}$ and minimize the denoising score matching objective \cite{Song2020ScoreBasedGM}:
\begin{equation}\label{eq:loss}
    \lambda\big(\sigma(t)\big)||D_{\theta}(\tau_{gt}+\epsilon; s, \sigma) - \tau_{gt}||^2_2
\end{equation}
where $\lambda\big(\sigma(t)\big) = \frac{\sigma(t)^2+1}{\sigma(t)^2}$ weights the loss for a given noise level. $P_{mean}, P_{std}$ are scalar hyperparameters which we set to $-1.2$ and $1.2$ respectively, following \cite{Karras2022ElucidatingTD}.

During inference, we substitute Equation \ref{eq:solution} into Equation \ref{eq:ode} and solve by numerical integration using Heun's second-order method \cite{Karras2022ElucidatingTD}. This is a deterministic sampler and amounts in taking $N$ finite steps corresponding to time steps $t_0, t_1, \dots , t_N$, where $t_N = 0$.   We explain the inference process in more detail in Section \ref{sec:inference} of the appendix.


\paragraph{Policy encoder}
We discuss now our design of the function $F_{\theta}$, as well as the state representation $s$. We base our architecture on Urban Driver \cite{Scheel2021UrbanDL} and extend it to support iterative denoising as a diffusion model. Specifically, the agents and road segments are featurized with separate MLPs to obtain a set of agent and road tokens that constitute the state. We encode a noisy trajectory with a separate MLP to obtain a sequence of trajectory tokens. The different tokens are concatenated to form a long sequence of trajectory, road and agent tokens. We also add a learnable type embedding to each token to indicate whether it is a trajectory token, road token, agent token or the specific ego vehicle token. Since diffusion models need to condition on the denoising timestep as well, we encode $\sigma(t)$ with an MLP and add the resulting vector to all tokens. 
The formed token sequence is fed to a transformer with $8$ self-attention layers \cite{DBLP:journals/corr/VaswaniSPUJGKP17} that contextualizes the token set. The updated trajectory tokens are fed to an MLP to regress the denoised trajectory and update our current estimate using Equation \ref{eq:network}.

\subsection{Controllable trajectory generation} \label{sec:controlability} 

% How we get the diffusion model to follow points
Prior work \cite{janner2022planning,MotionDiffuser} has shown that diffusion models can perform guided sampling using arbitrary cost functions at test-time without retraining.
This is equivalent to sampling from the joint distribution $p(\tau | s) q(\tau|s)$, where $p(\tau | s)$ is our inferred distribution over future trajectories and $q(\tau | s)$ is some constraint manifold.
The score function for this joint distribution can be decomposed as:
\begin{equation}
    \nabla_\tau \log \big( p\big(\tau; s, \sigma(t)\big) q\big(\tau; s, \sigma(t)\big) \big) = \nabla_\tau \log p\big(\tau; s, \sigma(t)\big) + \nabla_\tau \log q\big(\tau; s, \sigma(t)\big)
\end{equation}
which means we only need to estimate the constraint gradient score $\nabla_\tau \log q\big(\tau; s, \sigma(t)\big)$ to perform constrained sampling.
\cite{MotionDiffuser} approximates the constraint gradient score for some arbitrary cost function $\mathcal{L}$ and penalty weight $\lambda$ as follows:
\begin{equation}\label{eq:q_score}
    \nabla_\tau \log q\big(\tau; s, \sigma(t)\big) \approx \lambda \frac{\partial}{\partial \tau} \mathcal{L} \big( D_{\theta}\big(\tau; s, \sigma(t)\big) \big)
\end{equation}
In order to do controlled sampling, we adopt a modified version of the attractor cost function introduced in \cite{MotionDiffuser}, which penalizes deviation from some goal trajectory.
Specifically, we penalize the distance between each waypoint in $\tau \in \mathbb{R}^{Tx2}$ and some goal point $g \in \mathbb{R}^{2}$.
While \cite{MotionDiffuser} penalizes the distance from the goal waypoint to only the final point of the predicted trajectory, we penalize the distance to all points and introduce exponential weighting to decrease the penalty incurred for earlier points:
\begin{align*}
    \mathcal{L}(\tau; g) &= \sum_{t} w_{t} || \tau_{t} - g || \\
    w_{t} &= e^{b(\frac{t}{T}-1)}
\end{align*}
where $b$ is a tunable parameter controlling the rate of exponential decay (for our experiments we find $b=2$ to work well).
Note that this formulation can also be inverted to guide predictions away from specific points.

\paragraph{Mapping driving instruction to programs with LLM prompting}
%
%For the language-guided diffusion policy trajectories, \model{} 
We prompt GPT-4 \cite{gpt4} to parse instructions to python programs that, when executed, output cost maps to guide ego-vehicle trajectory generation. % using GPT-4 \cite{gpt4}.  %trained on extensive internet-scale language data. 
%These models are utilized to direct trajectories towards goal states instructed by language.
%To accomplish this, the model is provided with
Our prompt design is inspired by Code-as-Policies  \cite{liang2022code}. It begins by importing commonly used Python libraries that contain functions for comparisons and arithmetic operations, such as NumPy and Shapely. It then includes a list of API functions  for accessing the current state of the environment. Following this, we provide several examples where the task is communicated as Python comments, along with the corresponding code output that we have written. We append the new task we desire the output for as a comment directly after the prompt. The Language Model then generates the desired Python code output based on this prompt.
The prompt used is depicted in Figure \ref{fig:prompt}, and the associated output generated by the Language Model is presented in Figure \ref{fig:output_llm} of the appendix.  

%Our prompt 
%language instructions and has access to 
%includes a list of API functions that can retrieve the current state of the environment, such as the position of the driving vehicle, other vehicles, lanes, stop signs, pedestrians, etc. 

%The objective of the Language Model is to produce Python code that, upon execution, provides the coordinates of points that are ideal for reaching the goal or points that the car's trajectory should avoid. 

%These tasks may also require closed-loop feedback, such as waiting for the car in the left lane to pass before changing lanes. In such scenarios, the Language Model generates Python code that continuously interacts with the environment through the given API, querying its state and issuing commands at each time step to guide the car's actions.

%We adopt the Code-as-Policies approach \cite{liang2022code} for prompting the Language Model \cite{Chen2021EvaluatingLL}.

%We also provide a few examples that utilize the provided API functions as prompts, we enable the Language Model to perform various language tasks, as discussed in our experiments. 



%To design the prompt, we begin by importing commonly used Python libraries that contain functions for comparisons and arithmetic operations, such as NumPy and Shapely. Additionally, we import domain-specific functions that serve as an API for accessing the current state of the environment. Following this, we provide several examples where the task is communicated as Python comments, along with the expected code output that we have written. We append the new task we desire the output for as a comment directly after the prompt. The Language Model then generates the desired Python code output based on this prompt.

% \todo{AYUSH-BRIAN}
%\subsubsection{Augmenting demonstration trajectories}


% \paragraph{Implementation details} 
% While some methods predict steering angles directly, predicting waypoints allow policies to generalize across different ego-vehicle dynamics \cite{modularity}. 
% Following \cite{LAV,plant}, we use a PID controller to move the vehicle from one waypoint to the next. 
% %A well-known problem with behavior cloning methods is distribution mismatch between the state distribution of the demonstrator and the state distribution the policy will encounter during deployment. Small mistakes of the learnt policy will send the agent to states where it does not know  how to recover \cite{dagger}. To handle error compounding 
% We augment the training demonstrations, as shown in Figure \ref{fig:augmentations}. We find it useful to apply a linearly decaying lateral translational offset to the ego-trajectory. This does not affect the final position of the predicted trajectory, which allows the model to learn corrective behaviors without erroneous targets. Additionally, we randomly rotate the scene $\pm10^{\circ}$ around the ego-vehicle. 
%To our surprise, we find that dropping out random agents from the scene graph actually hurts performance and would cause the agent to freeze. We suspect that this is because removing arbitrary agents from the scene may actually change the optimal future trajectory in some cases. For instance, if we remove the leading vehicle our demonstrator is stopping for, then our agent may learn to stop for non-existent cars.

%We noticed that  state-based methods that condition on  dense sub-goal waypoints do not train with augmentations \cite{plant}. We hypothesize that this is due to significantly reduced compounding errors when allowed access to dense sub-goal waypoints.  We show experimentally that the use of data augmentations is critical to strong performance when we do not have access to this privileged route information. 

% maybe this isn't worth including, but in case we need space i feel like this was an interesting observation


==> OLDmethod2.tex <==

\begin{figure*}[h!]
  \centering
    \includegraphics[width=0.975\linewidth]{figures/arch.pdf}
  \caption{\textbf{Diagram for \model{}.} We visualize our diffusion guidance procedure. Trajectories are colored by rewards (blue is lower, green is higher).\todo{replace place holders in the denoising process}
  }
  \label{fig:architecture}
\end{figure*}



\section{Method}  \label{sec:method}


% The architecture of \model{} is shown in Figure \ref{fig:architecture}. 
% We describe background material on evolutionary methods and diffusion models in \ref{sec:background}. We describe \model{} in Section \ref{sec:ourmodel} and its application on instruction following in  %optimizing  controllability from language instructions in
% Section \ref{sec:lang}. %language-controllable trajectory generation in the following subsections.

\subsection{Background} \label{sec:background}

\paragraph{Diffusion models}
% \todo{tw: very similar to 3D diffuser actor}A diffusion model learns to model a probability distribution $p(x)$ by inverting a process that gradually adds noise to a sample $x$, which is known as the forward diffusion process. 
% The amount of noise added varies according to the diffusion timestep $t$ following a variance schedule of $\{\beta_t \in (0,1)\}_{t=1}^{T}$. Forward diffusion process adds noise to $x$ following $x_t = \sqrt{\bar{\alpha}_t} x + \sqrt{1-\bar{\alpha}_t} \epsilon$ where
% $
% \epsilon \sim \mathcal{N}(\bzero,\bone),
% $
% is a sample from a Gaussian distribution (with the same dimensionality as $x$), $\alpha_t = 1- \beta_t$, and $\bar{\alpha}_t = \prod_{i=1}^t \alpha_i$.  It then learns a reverse diffusion process that predicts the noise $\hat \epsilon$ given $x_t$ and $t$ as input
% The denoising process is modeled by a neural network 
% $ \hat \epsilon = \epsilon_{\theta}(x_t;t) $ 
% that takes as input the noisy sample $x_t$ and the noise level $t$ and tries to predict the noise component $\epsilon$. 

% In order to draw a sample from the learned distribution $p_\theta(x| \cond)$, we start by drawing a sample $x_T \sim\mathcal{N}(\mathbf{0},\mathbf{1})$. 
% Then, we progressively denoise the sample by iterated application of $\epsilon_{\theta}$ according to a specified sampling schedule \cite{ho2020denoising,song2020denoising}, which terminates with $x_0$ sampled from $p_\theta(x)$.

A diffusion model captures the probability distribution $p(x)$ through the inversion of the forward diffusion process, that gradually adds Gaussian noise to the intermediate distribution of a initial sample $x$.  The amounts of added noise depend on a predefined variance schedule ${\beta_t \in (0,1)}_{t=1}^{T}$, where $T$ denotes the total number of diffusion timesteps.  At diffusion timestep $t$, the forward diffusion process adds noise into $x$ using the formula $x_t = \sqrt{\bar{\alpha}_t} x + \sqrt{1-\bar{\alpha}_t} \epsilon$, where $\epsilon \sim \mathcal{N}(\bzero,\bone)$ is a sample from a Gaussian distribution with the same dimensionality as $x$. Here, $\alpha_t = 1- \beta_t$, and $\bar{\alpha}t = \prod{i=1}^t \alpha_i$.  For denoising, a neural network $\hat \epsilon = \epsilon_{\theta}(x_t;t)$ takes input as the noisy sample $x_t$ and the diffusion timestep $t$, and learns to predict the added noise $\epsilon$.  %Here, we consider conditional diffusion models to capture a distribution $p(x|\cond)$ conditioned on input $\cond$.  The denoising network $\hat \epsilon = \epsilon_{\theta}(x_t, c;t)$ thus takes additional input as $\cond$.

To generate a sample from the learned distribution $p_\theta(x)$, we start by drawing a sample from the prior distribution $x_T \sim \mathcal{N}(\mathbf{0},\mathbf{1})$ and iteratively denoise this sample $T$ times with $\epsilon_\theta$.  The application of $\epsilon_\theta$ depends on a specified sampling schedule~\cite{ho2020denoising,song2020denoising}, which terminates with $x_0$ sampled from $p_\theta(x)$.

% \todo{in DDPM they have this formulation: $p_\theta (x_0) := \int p_\theta (x_{0:T}) dx_{1:T}$}
% : %. The iterative denoising 
% \begin{equation} \label{eq:diffupdate}
% \nonumber
% x_{t-1} = \frac{}{\sqrt{a_{t}}} \left( x_t - \frac{\beta_t}{\sqrt{1-\bar{\alpha}_t}} \epsilon_\theta (x_t,t,\cond) \right) +\sigma_t \mathbf{z}, \text{   where    } \mathbf{z} \sim \mathcal{N} (\bzero,\bone) 
% \end{equation}

\paragraph{Conditional generation with diffusion models}
% Substantial effort has been devoted towards conditional sampling with diffusion models.
Diffusion models can be easily extended to model $p(x|\cond)$, where $\cond$ is some conditioning signal, such as the expected future rewards or some language instruction, by adding an additional input to the denoising neural network $\epsilon_{\theta}$.
However, this relies on having labeled conditions in our training dataset, which can be prohibitively expensive to generate when dealing with real-world datasets.
This also scales poorly with the complexity of the conditioning information -- we need more data to ensure good coverage as the dimensionality of our input features increases.
Additionally, it can be challenging for these approaches to generalize to novel sample-context pairs.

Prior work \cite{janner2022planning,MotionDiffuser} has shown that diffusion models can perform guided sampling using arbitrary reward functions at test-time without retraining.
Practically, this involves maximizing a differentiable reward function w.r.t $x$ by alternating between reward gradient steps and denoising steps during inference.
However, this approach requires us to have a reward function which is both differentiable and able to handle noisy samples since it is used during the denoising process.
It can also be challenging to balance the trade-off between adherence to the conditioning input and the base diffusion model.
For large guidance weights, sampling can be unstable due to samples being pushed too far from the data manifold.

% This is equivalent to sampling from the joint distribution $p(\tau | s) q(\tau|s)$, where $p(\tau | s)$ is our inferred distribution over future trajectories and $q(\tau | s)$ is some constraint manifold.
% The score function for this joint distribution can be decomposed as:
% \begin{equation}
%     \nabla_\tau \log \big( p\big(\tau; s, \sigma(t)\big) q\big(\tau; s, \sigma(t)\big) \big) = \nabla_\tau \log p\big(\tau; s, \sigma(t)\big) + \nabla_\tau \log q\big(\tau; s, \sigma(t)\big)
% \end{equation}
% which means we only need to estimate the constraint gradient score $\nabla_\tau \log q\big(\tau; s, \sigma(t)\big)$ to perform constrained sampling.
%In  denoising diffusion implicit models (DDIMs) \cite{DDIM}, there is no added noise in intermediate steps, and the only stochasticity in sampling comes from the initially sampled noise  $x_T \sim\mathcal{N}(\mathbf{0},\mathbf{1})$:
%\begin{equation} \label{eq:diffupdate}
%x_{t-1} = \frac{}{\sqrt{a_{t}}} \left( x_t - \frac{\beta_t}{\sqrt{1-\bar{\alpha}_t}} \epsilon_\theta (x_t,t,\cond) \right).
%\end{equation}

\paragraph{Evolutionary strategies}
As opposed to gradient-based optimization methods which are commonly used for diffusion guidance, evolutionary strategies are a family of population-based \textit{gradient-free} optimization algorithms which can maximize arbitrary black-box reward functions without any offline training.
In ES, our objective is to maximize some reward (or fitness) function $R(x) : \mathbb{R}^{d} \rightarrow \mathbb{R}$ where $x$ is our decision variable.
During optimization, we iteratively update a search distribution $q(x)$ to maximize expected rewards $\mathbb{E}_{x\sim p_{\theta}(x)}[R(x)]$.
While distribution-based ES approaches such as CEM and CMA-ES represent $q(x)$ explicitly (often as a unimodal Gaussian), we can also represent $q(x)$ non-parametrically as a set of high-performing solutions without making strong assumptions about the functional form of $p_\theta$.

The optimization loop proceeds as follows.
First, we generate a population of samples $\{x_i\}$ by sampling from our search distribution $x_i \sim p_{\theta}(x)$. 
Next, each sample is evaluated using with our reward function $R(x)$. Note that this only requires the ability to query $R(x)$ and does not require differentiability.
Lastly, we update $\theta$ using the highest performing samples. The sampling and update formulations are dependent on how $p_{\theta}$ is parameterized and the specific algorithm being used. 
% For instance in CEM, the top $K$ samples are selected and used to fit a Gaussian which is our updated $q$, which can be used for sampling at the next iteration. 
In classical population-based ES, the population at the next iteration consists of mutated copies of the current top $K$ samples, where mutations are performed by perturbing $x$ with random noise.
This loop is repeated to iteratively refine $p_\theta$.

\subsection{Diffusion Evolutionary Search} \label{sec:ourmodel}

% % ES perspective -- use learning to accelerate optimization by pushing samples to the true data manifold
% One major challenge with ES is intelligent exploration.
% Random noise perturbations are a highly inefficient way of exploring the solution space.
% While they may be suitable for black-box objectives where we have minimal prior information, ideally we would be able to use our diffusion model to push candidates towards the true data manifold.
% % Diffusion perspective -- how do we constrain ES so it doesn't deviate from our model support
% Another perspective on the same problem is that in order to use ES for guided sampling, we must ensure that the search distribution $p_\theta$ does not deviate too far from the training distribution of our model.

Now we present \model{}, our novel guidance approach which leverages evolutionary search to perform guided sampling from trained diffusion models.
Specifically, we use a learned diffusion model to initialize the population and project mutated samples onto the data manifold.
The overall method is visualized in Figure \ref{fig:architecture} and Algorithm \ref{alg:diff-tta}.

\paragraph{Initializing the population with diffusion samples}
We begin by sampling an initial population $X^{0}$ of $M$ samples using our diffusion model:
\begin{align}
    X^{0} = \{ x_{i}\}_{i=1}^{M} \sim p_{\theta}(x)
\end{align}
where $X^{k}$ is the population at iteration $k$.
This involves a complete pass through the reverse diffusion process.
We can flexibly modify the initial population to bias our sampling, e.g. by including samples generated by other approaches or mixing in solutions from the previous timestep to warm-start our optimization.

\paragraph{Sample scoring}
At each iteration $k$ we compute rewards $\{ R(x_{i}) | x_{i} \in X^{k}\}_{i=1}^{M}$ across the entire population, where $R(x)$ can be any black-box reward function.
Note that our population consists of "clean" samples so we do not need an objective which can handle "noisy" samples, which gives us significant flexibility compared to guidance methods that perform classifier-based guidance.

\paragraph{Selection}
We use rewards to decide which samples we should select to propagate to the next iteration.
Following MPPI \cite{williams2015model}, we resample $X^{k+1}$ proportional to $R(x)$:
\begin{align}
    q(x) &= \frac{\exp (\tau R(x))}{\sum_{i=1}^{M} \exp (\tau R(x_i))} \\
    E^{k+1} &= \{ x_{i} \overset{\mathrm{iid}}{\sim} q(x)\}_{i=1}^{M}
\end{align}
where $E^{k+1}$ represents our elite set which is kept from iteration $k$, and $\tau$ is a tunable temperature parameter controlling the sharpness of $q$.
% We consider two simple strategies inspired by CEM and MPPI, which are both popular ES variants:
% \begin{enumerate}
%     \item \textbf{CEM}: We select the $K$ samples with the highest rewards to be our elite set. We then resample our population uniformly from this elite set \todo{math}
%     \item \textbf{MPPI}: We resample our population from all samples proportional to rewards \todo{math}
% \end{enumerate}
% We find that these two methods perform similarly, so we use the MPPI-variant for our experiments.

\paragraph{Mutation using truncated diffusion}
We apply randomized mutations to $E^{k+1}$ to encourage exploration.
For black-box optimization, prior ES methods resort to naive Gaussian perturbations which do not exploit any prior knowledge about the solution space.
Our key insight is that we can leverage our diffusion model to guide candidate trajectories towards the data manifold by using a truncated diffusion process.
We can run the first $t$ steps of the forward diffusion process to get noised elite samples $\bar{E}^{k+1}$:
\begin{align}
    \bar{E}^{k+1} = \{\sqrt{\bar{\alpha}_N} x + \sqrt{1-\bar{\alpha}_N} \epsilon | x \in E^{k+1} \}
\end{align}
where $\epsilon \sim \mathcal{N}(\bzero,\bone) $.
Then we can run the last $t$ steps of the reverse diffusion process to denoise the samples again, giving us clean samples $X^{k+1}$:
\begin{align}
    X^{k+1} = \{x \sim p_\theta(x | \bar{x}) | \bar{x} \in \bar{E}^{k+1}\}
\end{align}

Depending on the scale of the Gaussian noise added, we only need to run a small fraction of the total number of denoising steps used to synthesize samples from scratch.
This allows us to incorporate prior information in our learned diffusion model without the computational cost of running the full reverse diffusion process.
In practice, the number of timesteps $t$ of the truncated diffusion process is a tunable time-dependent hyperparameter $t_k$ which controls the mutation strength at each iteration $k$.

\paragraph{Implementation details}
In our experiments we use a population size of $M=128$.
Our diffusion model is trained with $T=100$ denoising steps.
We find that linearly decaying the number of mutation diffusion steps $t_k$ from 5 to 1 over 20 search steps works best in our experiments.

\begin{figure*}[h!]
  \centering
    \includegraphics[width=0.975\linewidth]{figures/instructions.pdf}
  \caption{\textbf{Shaping reward functions with language using LLM prompting.} 
  We show initial scene and cost map and solution found by \model{}. We show the resulting reward function using language instruction and the altered behaviour generated by \model{}.
  }
  \label{fig:lang}
\end{figure*}

% \todo{BRIAN FIX ALGO}
\begin{algorithm}[H]
   \caption{$\texttt{\model{}}$}
   \label{alg:diff-tta}
\begin{algorithmic}[1]
    \STATE {\bfseries Input:} Diffusion model $p_\theta$, reward function $R$, search steps $K$, population size $M$, number of noising steps $N$, variance schedule $\bar{\alpha}=\{\bar{\alpha}_i\}_{i=1}^N$.
    \STATE {\bfseries Initial proposals:} $X^0 \leftarrow \{x_i \sim p_\theta (x)\}_{i=1}^M$
    \FOR{search step $k \in (1, \dots, K)$}
        \STATE Score proposals $\{R(x_i) | x_i \in X^{k-1}\}_{i=1}^M$
        \STATE Compute distribution $q (x)=\frac{\exp(R(x))}{\sum_{i=1}^{M} \exp(R(x_i))}$
        \STATE Sample elites from $X^{k-1}$: $E^{k} \leftarrow \{x_i \overset{\mathrm{iid}}{\sim} q(x)\}_{i=1}^M$
        \STATE Renoise elites
        $\bar{E}^{k} \leftarrow \{\sqrt{\bar{\alpha}_N} x + \sqrt{1-\bar{\alpha}_N} \epsilon | x \in E^k , \epsilon \sim \mathcal{N}(\bzero,\bone) \}$
        \STATE Denoise elites $X^{k} \leftarrow \{x \sim p_\theta(x | \bar{x}) | \bar{x} \in \bar{E}^k\}$
    \ENDFOR
    \RETURN output $x = \argmax_{x \in X^K} R(x)$
\end{algorithmic}
\end{algorithm}


\subsection{Mapping language instructions to reward functions with LLM prompting} 
\label{sec:lang}
In this section, we show how we map language instructions to black-box reward functions which we optimize with \model{}.  
%\paragraph{Synthesizing reward code from instructions}
We adopt a similar approach to \cite{yu2023language} which uses LLMs to synthesize reward functions from language instructions. 
%We find that reward function code is an intuitive interface for controlling driving policies for several reasons.
%Since urban driving environments are highly stochastic and require interacting with other dynamic agents, we cannot rely on executing open-loop primitives.
Reward functions are composable and allow us to seamlessly combine language guidance with other constraints.
This is crucial in driving where we are constantly optimizing many different objectives at once (e.g. safety, driver comfort, route adherence).

%\paragraph{Closed-loop instruction guidance with Python generators}

\cite{yu2023language} produces a stationary reward function, i.e. one which is fixed during planning.
We note that in many situations, this can make it challenging to express sequential plans solely through rewards. 
For an instruction such as "Change lanes to the left, then pass the car on right, then take the exit", we would need to introduce several auxiliary state variables to encode this behavior following the approach in \cite{yu2023language}.
We find that a much more natural and succinct way of capturing these plans in code is through the use of \textit{generator functions} which retain internal state between calls.
Code examples can be found in Figure \ref{fig:lang} and in the supplement.

%\paragraph{Language-augmented reward functions}
Similar to prior work, we expose a Python API which can be used to extract information about entities within the scene and the road graph.
Since many of the basic reward signals in driving do not change from scenario to scenario (e.g. collision avoidance, drivable area compliance), we allow the LLM to write \textit{reward augmentation} code which modifies the behavior of the base reward function.
Augmentations can add auxiliary reward terms (e.g. a dense lane-reaching reward) or re-weight existing reward terms.
In the next section, we show how these language-augmented reward functions can be used to synthesize rich and complex driving behaviors.

% Our prompt design is inspired by Code-as-Policies  \cite{liang2022code}. It begins by importing commonly used Python libraries that contain functions for comparisons and arithmetic operations, such as NumPy and Shapely. It then includes a list of API functions  for accessing the current state of the environment. Following this, we provide several examples where the task is communicated as Python comments, along with the corresponding code output that we have written. We append the new task we desire the output for as a comment directly after the prompt. The Language Model then generates the desired Python code output based on this prompt.

% %The prompt used is depicted in Figure \ref{fig:prompt}, and the associated output generated by the Language Model is presented in Figure \ref{fig:output_llm} of the appendix.  


% Our LLM prompts %to generate task descriptions, task decompositions and rewards functions 
% contain the following sections: 
  

% \noindent \textbf{2. Instructions.}  These  include function APIs that can be used by the LLM to query the pose of the robot end-effector, as well as different assets in the given environment:

% \lstinputlisting[language=Python]{code/reward.py}

% \noindent \textbf{3. Examples of task descriptions and decompositions.} These are question-answer pairs that demonstrate task descriptions and their temporal decompositions. %of how tasks can be decomposed into subtasks.
% %language questions can be answered for task decomposition and reward generation.  % can be mapped into code. Examples for task decomposition into subtasks 

% \lstinputlisting[language=Python]{code/reward.py}

% \noindent \textbf{4. Examples of reward functions.} These are task to reward function pairs that present demonstrations of how tasks can be translated to reward functions, as shown below: 
% %as well as reward functions for each subtask. 
% %\begin{equation}
% %\label{eq:reward}
% %\lambda_d R_{\text {dist}}+\lambda_p R_{\text {pose}}+\lambda_t R_{\text {grasp}}
% %\end{equation}
% %Note that the following is just an example for the LLM to use as a reference.
% \lstinputlisting[language=Python]{code/reward.py}
% For the example above, the  reward function is  comprised of 1) distance between the end-effector and the target part, and 2) distance between the current and the target pose of an articulated asset, link, or joint. 

==> driving_setup.tex <==
Now we present our planning setup in nuPlan.
We train our diffusion model on an offline dataset of 250K driving trajectories.
Trajectories are predicted 8s into the future at 2Hz, corresponding to 16 predicted future waypoints.

To perform planning, we need a reward function $R(x)$ which scores a predicted driving trajectory $x$ directly.
We adopt a similar approach to PDM-Closed \cite{dauner2023parting} which rolls out driving trajectories in an internal world model and then scores them using manually defined planning costs, e.g. progress along route, drivable area compliance, driver comfort, etc.
Vehicle kinematics are simulated using a bicycle model and the behavior of other dynamic actors is estimated using heuristics such as assuming constant velocity.

Since our guidance method does not assume differentiability, we can directly optimize $R(x)$ independent of how this internal world model is implemented.
Note that differentiating through $R(x)$ in this instance is challenging due to the use of non-differentiable heuristics used to simulate actors and the use of highly non-smooth planning costs (e.g. collisions).


==> notes.tex <==

Notes:
We need to justify: why we need language? Why the vanilla reward doesnt suffice for driving?

==> oldabstract.tex <==



\begin{abstract} 
We marry evolutionary  search  with  generative modelling  for trajectory optimization. Evolutionary  search methods such as CEM and MPII,   iteratively sample and score trajectory proposals to optimize  black-box cost functions and are ubiquitous in robot trajectory planning. 
However, they %do not benefit from trajectory samples to learn sampling from the data manifold and 
%model cannot efficiently sample trajectories from the data trajectory manifold and 
%as a result 
they waste compute on scoring unnatural, infeasible or uncommon samples since they cannot efficiently sample from the  trajectory data manifold. 
 %trajectory samples lying far from the data  manifold as they do . 
 Reward guided diffusion-based  trajectory sampling can generate trajectories that both belong to a trajectory manifold, captured by a diffusion model, and maximize a differentiable reward function, by alternating between diffusion denoising steps and reward gradient steps. The reward function needs to be differentiable and fitted on both clean and noised samples, which limits their generality. In this paper, we propose \model{}, an evolutionary method that  can optimize arbitrary non-differentiable black-box objectives without retraining by sampling  trajectory proposals using a truncated reverse diffusion process that noises and denoises trajectories. It significantly accelerates optimization thanks to focusing computation on  samples that belong to the trajectory data manifold. Because our trajectory  mutation process only uses a small number of noising and denoising steps, it is computationally feasible and not slower than original ES methods. We test \model{} in driving and  instruction following in nuPlan, an established benchmark for autonomous driving. We show it generates safe and compliant driving behaviors on a suite of challenging planning tasks, and outperforms both sampling-based planners and reward-guided diffusion sampling. For instruction following, we use few-shot LLM prompting to map language instructions to programs that shape the reward function optimized by \model{} and baselines. %, and control behaviour of the driving agent. 
%We validate our results in nuPlan and show that our approach can generate safe and compliant driving behaviors on a suite of challenging planning tasks. 
\model{} can effectively optimize the generated reward functions from  general language instructions and generate highly complex behaviors, such as aggressive lane weaving,   not present in the training data, and 
%. Finally, we show that our planner can be used to 
solve the hardest nuPlan scenarios through language feedback from a human expert, while other planners or reactive driving policies fail to do so.
%trajectory sampling that combines the best of evolu
%They do not improve with more data and ths
%In this paper, we use diffusion models to perform language-guided closed-loop planning for autonomous driving. Conventional wisdom suggests one can use scene-conditioned diffusion policies with classifier guidance to flexibly plan over novel objectives at test-time. We show that excessive conditioning information can hinder downstream planning performance due to poor generalization and lack of diversity. Additionally, we show that gradient-based optimization (e.g. classifier guidance) can actually perform worse than sampling-based optimization (e.g. CEM/ES) for guided diffusion sampling at lower dimensionality, which we show experimentally. To that end, we demonstrate how a diffusion model with no conditioning information at all can be used to accelerate planning using online sampling-based guidance. We introduce a novel sampling-based guidance method DiffusionES which handles arbitrary non-differentiable black-box objectives without retraining. DiffusionES uses a truncated reverse diffusion process to denoise candidates which significantly accelerates optimization. We use LLMs to map language instructions to programs which adaptively control the behavior of our planner through reward shaping. We validate our results in nuPlan and show that our approach can generate safe and compliant driving behaviors on a suite of challenging planning tasks. Additionally, with language supervision our approach can synthesize highly complex behaviors (such as aggressive lane weaving) which are not present in the training data. Finally, we show that our approach can be used to solve the hardest nuPlan scenarios through language feedback from a human expert.
% We marry diffusion-based  generative models with zero-shot instruction-to-program generation with  Large Language Models (LLMs). We propose   a diffusion-based driving policy    that conditions on a tokenized  representation of the dynamic visual scene  and, optionally, a language instruction, and predicts a distribution over driving trajectories that follow traffic rules as well as the language instruction, when possible.  
% %for predicting a distrubution over car wayp
% %We propose a scene-conditioned trajectory diffusion policy, we call \model{}, for autonomous driving that  conditions on a tokenized scene representation of the dynamic visual scene, a far destination goal,  and, optionally, a language command, and predicts a driving trajectory that drives to the goal destination, following the language instruction if possible. 
% The model is trained from driving demonstrations to denoise noised vehicle trajectories, by attending to the scene context and a desired far destination goal. Our policy outperforms in driving ability its deterministic counterparts, as well as alternative trajectory generative policy formulations in the established nuPlan driving benchmark. 
% We show our policy can be controlled using natural language at inference time  zero-shot, without any additional training. Specifically, we prompt LLMs to map   language driving instructions to programs that output sets of waypoints on the road for the vehicle to reach or avoid. Inference in our diffusion policy using classifier-free guidance according to the program waypoint predictions 
% %We show  follows instruction in natural language by prompting Pretrained Large Language models to map language instructions to  programs that predict lanes and waypoints in the road for the vehicle to follow or avoid. 
% %The 
% controls the vehicle to change lanes, park behind another car,  change speed, keep distance from described landmarks, and combination of the above.   Handling multimodality in imitation learning for driving and following natural language  instructions are jointly handled in our diffusion-based formulation, thanks to the composability of diffusion generative models with additional constraints at inference time and their improved performance as  faithful generative models for modelling complex distributions. 

\end{abstract}



==> oldintro.tex <==
%\epigraph{Ask not what it is, ask what it is like.}{\textit{Moshe Bar}}

\section{Introduction}



\topic{what is trajectory optimization and how it is done with evolutionary search and what are the pitfalls}
Trajectory optimization searches for an action trajectory that minimizes a cost function subject to dynamics constraints, and it is a parsimonious procedure in reinforcement learning and control \cite{}. In the case of general dynamics models, such optimization cannot be obtained with a closed form solution, and it is often addressed with variants of evolutionary search, such as, cross entropy method (CEM) \cite{} or Path Integral Control (MPII) \cite{}. These are methods   that sample action trajectory proposals, score these  proposals using the designated cost function, and  sample new proposals in the vicinity of highest scoring ones. The fact that evolutionary algorithms does not need the cost function to be differentiable makes them general solvers across a wide variety of problems \cite{}. However, the process of sampling and mutating action trajectories is often quite naive and does not have general satisfying ways of sampling and mutating trajectories that being in the data trajectory manifold. Hand designed constraints are often used that are tailored to a specific problem and not general enough. In this way, a lot of computation is spent is sampling and scoring non realistic or natural action trajectories, making the search ineffective or suboptimal.



\topic{diffuser}
%Prior policies often guide the action sampling to accelerate such search \cite{}. 
Recent advances of generative modelling proposed a transformative way of interpreting trajectory optimization, by learning to sample from a trajectory manifold using trajectory diffusion model, and optimizing trajectories under a (differentiable) reward function by alternating between denoising generation steps and backpropagating reward gradients to the input action sequences \cite{}. In this way,  

%Conventional wisdom suggests one can use scene-conditioned diffusion policies with classifier guidance to flexibly plan over novel objectives at test-time.


%\topic{what is the role of industry and academia in driving, the fact that one has almost perfect perception, while the other only worries about training from pixels}
%\topic{}
Learning to drive from imitating  driving demonstrations is prevalent in the research and development of autonomous vehicles \cite{DBLP:journals/corr/abs-1710-02410,endtoendNVIDIA,gaildriving}.  %All methods 
Driving policies can take as input pixel and LiDAR input \cite{alvinn,endtoendNVIDIA,LBC,LAV,transfuser}, or use ground-truth perception of lanes, vehicles,  traffic signs and their  state attributes \cite{chauffernet,plant,roach}. In both cases, most methods predict  waypoints for the vehicle to follow, conditioned on a scene and a  distant goal representation. %Though learning from demonstrations is an established learning method, 
Most imitation learning methods optimize an objective that boils down to cloning the actions of the expert, as proposed  by Pomerleau decades ago \cite{alvinn}. Behaviour cloning has an underlying assumption of a unimodal Gaussian distribution for the actions to predict, which cannot handle  multimodality of  experts' driving behaviours, especially prevalent during accelerations, lane changes, merges, etc. . % Indeed, some many drive faster or slower, merge or bypass a car. %, and such multimodality cannot be adequately modelled by a unimodal Gaussian distribution.   
%hurts action regression, which is essentially what almost all methods have been using. 
%The limitations of behaviour cloning in the presence of multimodal action distributions is well documented in the literature \cite{}. 
Objectives and architectures that can better handle multimodal trajectory prediction have been  proposed,  
such as, mixture of expert  trajectory decoders \cite{wayformer}, combining classification and regression losses \cite{shafiullah2022behavior}, using Gaussian trajectory mixtures \cite{Kim_2023},   
conditional variational autoencoders (VAEs) with continuous or discrete latent variables \cite{multiplefutures, fragkiadaki2017motion}, producing heatmaps over a 2D bird's-eye-view  map to sample waypoint trajectories from \cite{lookout}. 

%\todo{??Most of them address offline trajectory forecasting and not closed loop control.} 
%In the recent nuPlan driving simuation benchmark the state-of-the-art using a GRU-based autoregressively predicted waypoints, similar to \cite{}, which is essentially a unimodal trajectory decoder. 

Parallely, controlling an autonomous vehicle in natural language will  enable  human passengers to influence the vehicle's route and behaviour beyond supplying a final goal destination. Passengers would be able to give feedback to the vehicle and suggest places to park, intermediate stops, vehicles to follow, lanes to prefer or change, or speed to use. Language controllability of an autonomous vehicle is important for versatility and personalization of the vehicle-human experience,  and for reinforcing trust and transparency  in human-vehicle interaction. 
% A vehicle would be expected to follow these instructions whenever possible, if traffic rules and safety permit.

%This poses the question

%control  be important for a user communicating its des

In this paper, we propose [model], a method for learning a driving policy from  demonstrations 
%while handling their multimodality, while also 
and controlling it in natural language. Our method marries diffusion-based  generative models for  trajectory prediction and large language models for  instruction-to-program generation. 
%We train a scene and goal conditioned transformer-based diffusion  policy from driving demonstrations. 
 Our policy attends on a variable-length tokenized representation of the scene in terms of static and dynamic entities, such as road lane points, vehicles,  bikers, traffic lights, as well as an approximate  indication of the  desired direction of the vehicle, and learns  to denoise noised  waypoint trajectories of the ego-vehicle. At inference time, we sample driving trajectories from the learnt distribution  by iteratively denoising  trajectories, following the continuous formulation of \cite{karras2022elucidating}.  
 %, namely, the vehicle that the policy controls.
%Our model %, and show it %obtains state-o-the-art performance, 
%outperforms the previous state-of-the-art in the recent NuPlan driving benchmark \cite{}. 
%We exploit the compositionality of diffusion to couple it
 We prompt LLMs to map language instructions to programs that ground  referential expressions to relevant scene entities and  output sets of  waypoints for the car to reach or avoid. 
 %,  using few-shot prompting of an LLM to ground  referential expressions to relevant entities and predict task-relevant landmarks the instruction directs.
 We couple trajectory sampling with language-instructed landmarks to reach or avoid at inference time, using classifier-free guidance. We show resulting trajectories follow the language instruction while obeying traffic rules. 


Our language controllability builds upon code-as-policies \cite{liang2022code} in that it  prompts LLMs to predict programs for parsing instructions. Instead of predicting coordinate locations for pick and place control primitives which directly  parametrize the robot actions, our model combines predicted waypoints with a trajectory diffusion model to predict actions that both comply with a trajectory prior and attempt to follow the instruction. In that sense, we do not expect the LLM to know how to drive; this is the responsibility of the driving diffusion model. The LLM is merely responsible for interpreting language as cost maps to guide trajectory diffusion sampling. For example, the instruction \textit{``merge in the left lane"} should predict a program that outputs low cost for all waypoints in the left lane; the one most suitable to reach based on the current velocity and scene context should be selected during guided trajectory diffusion sampling. 

%prompts the LLM to  predict  programs that outputs sets of waypoints that satisfy the constraint of the language instruction, and not a specific  to predict cost maps 


We test our method in NuPlan \cite{caesar2022nuplan},  a recent  benchmarks for driving. We show our diffusion driving policy  outperforms the previous state-of-the-art,  a deterministic  neural transformer, and alternative generative policy formulations. We show that despite our top-1 offline trajectory performance is lower than a deterministic driving policy, our driving performance is better by an absolute margin of \todo{6\%}. %Our experiments agree with observations in previous works that suggest that offline driving performance is not indicative of closed loop driving.
We then show extensive examples of language controllability of our policy, and quantify its performance. 
%Given that this task does not exist any baselines,  we introduce a related benchmark for comparisons with future work. 


Closest to our work are the recent method of \cite{controllabletraffic} and concurrent work of \cite{MotionDiffuser}. %While these methods 
%\todo{DETAILS:
They both show that diffusion models can be used for forecasting offline vehicle trajectories, and controlling  them via attracting them or repelling them from specific waypoints, or using cost maps related to traffic rules. % using classifier free guidance.} 
The methods are motivated by controllability of diffusion models at inference time. 
%Work of \cite{MotionDiffuser} further evaluates offline trajectory performance using minSADE, a top-6 trajectory matching metric, and shows state-of-the-art performance. 
%The proposed models do not outperform the previous work in offline trajectry prediction in the 
%None compares on estblished benchmarks  and not by improved offline trajectory performance. 
Our work is inspired by these works; instead of offline trajectory prediction it is the first to use diffusion policies for closed-loop driving and outperform previous formulations in nuPlan. %While in top-1 offline trajectory prediction error our method is worse than the baselines, it is able to better captures the trajectory distribution in rare  scenarios such as turns, leading in improved online driving performance. 
%Our experiments show that this is significant: the offline performance of diffusion policy was worse than existing deterministic alternatives. However, in rare scenarios critical for driving, diffusion better captures the trajectory distribution, leading in improved driving performance. 
Furthermore, we are the first to show language controllability of diffusion policies by marrying diffusion with LLM prompting for instruction-to-program generation. %\todo{++}


% \paragraph{Contributions}
Our contributions are as follows:
\begin{enumerate}
\item The first diffusion-based driving policy, with SOTA performance in an established driving simulation benchmark.
\item Language controllability of a diffusion-based policy zero shot, without any instruction-trajectory training pairs, based on LLM instruction-to-program generation.
\item Extensive comparisons with alternative formulations for driving performance and language controllability. 
%\item Introduction of a new dataset for language controllability of driving policies. ??
\end{enumerate}
Our code and models will become publicly available upon publication. 



%\begin{figure*}[t!]
%  \centering
%    \includegraphics[width=0.95\linewidth]{figures/intro_fig_small.png}
%  \caption{} 
%  \label{fig:intro}
%\end{figure*}




==> oldrelated.tex <==
\section{Related work}
% \todo{to cite VoxPoser}
% AdaptDiffuser: Diffusion Models as Adaptive Self-evolving Planners


\paragraph{Diffusion models for decision-making and trajectory optimization} Diffusion models \cite{SohlDickstein2015DeepUL,ho2020denoising,song2020denoising,nichol2021improved} learn to approximate the data distribution through an iterative denoising process and have shown impressive results on image generation \cite{Dhariwal2021DiffusionMB,Saharia2022PhotorealisticTD,Rombach2021HighResolutionIS,Ramesh2022HierarchicalTI}. 
They have been used for imitation learning for manipulation tasks \cite{chi2023diffusion,reuss2023goal,pearce2023imitating,XianChainedDiffuserUT}, for controllable vehicle motion generation \cite{Zhong2022GuidedCD,Jiang_2023_CVPR,Carvalho2023MotionPD} and for video generation of manipulation tasks \cite{Du2023LearningUP,Yang2023LearningIR}. 
%Their main advantage is that they can better capture the action trajectory distribution compared to previous  generative models. 

In this work,  we explore their performance in learning to drive from demonstrations, as well as their controllability from language instructions.

% \paragraph{Guided diffusion sampling for planning and control}
% While diffusion policies have seen widespread use in many control applications, controllable planning with diffusion models remains relatively under-explored.
% Many approaches that perform guided diffusion sampling for control directly apply techniques that have seen widespread use in other domains.
% As mentioned previously, many approaches \cite{janner2022diffuser, liang2023adaptdiffuser, Carvalho2023MotionPD} train a reward classifier which can be used to guide sampling by maximizing rewards directly with gradient-based optimization, which is akin to classifier guidance.
% \todo{Not sure how much to discuss this since the intro focuses on this too}.

% With growing attention being paid towards scaling up large multimodal offline datasets across a variety of domains such as manipulation and autonomous driving, we see conditional generation from generative models trained on such large offline datasets as an important area of need which our method addresses.


% Diffuser is the big one, closely related is AdaptDiffuser
% DecDiffuser is worth mentioning


\paragraph{Learning versus Planning for Autonomous Driving}
% Learning to drive from demonstrations 
% in an end-to-end manner has seen a resurgence in recent years \cite{DBLP:journals/corr/abs-1710-02410,endtoendNVIDIA,gaildriving}. Imitation learning methods  train neural network policies to map input to car waypoint trajectories \cite{endtoendNVIDIA}. 
% Sensor-based  methods take as input images and, optionally,  LiDAR sensor readings \cite{neat,LBC,LAV},  while state-based methods take as input oracle perceptual representations represented as rasterized BEV maps of lane, vehicle and traffic sign information \cite{chauffernet,roach},  %perspective semantic segmentation maps \cite{modularity},
% or as scene token graphs 
% %as input to graph neural networks or transformer networks
% \cite{plant}; our model belongs to this last category. %Driving benchmarks exist for both sensor-based and state-based methods. For example, the CARLA benchmark \cite{CARLA} is focused on learning to drive from sensory input, while NuPlan, which we use, focuses on driving from tokenized scene representations \cite{caesar2022nuplan}. 
% Methods that drive from pixels address the problem in its total complexity but  confound  perceptual mistakes with behavioural mistakes:   it is not easy to attribute driving failures to perceptual mistakes or to behavioural ones, due to the black box nature of neural networks. On the contrary, state-based  methods isolate perception from behaviour and demonstrate what can be achieved with oracle perception, and what behavioural mistakes still need to be addressed. 




%Recent work by Chen et al. (2015) demonstrated a convolutional net to estimate affordances such as distance to the preceding car that could be used to program a controller to control the car on the highway.
%Bojarski et al. \cite{endtoendNVIDIA} showed how to train a deep convolutional neural network from driving demonstrations to  steer a car by consuming camera input. 
%A three-camera rig was used to automatically generate augmentation data, in the form of images paired with recovering steering actions from the left and right cameras. 
%Kuefler et al. \cite{gaildriving} use Generative Adversarial Imitation Learning (GAIL) as an alternative to augmentations to overcome cascading errors typically present in behavior cloned policies  so that they are more robust to perturbations. 
%Codevilla et al. \cite{DBLP:journals/corr/abs-1710-02410}  train a network using camera inputs and conditioned on high-level commands to output steering and acceleration. 


%Some 



%Driving simulator environments and benchmarks, such as the CARLA simulator \cite{CARLA}, have enabled research on  neural driving policies trained and deployed in simulation, as well as  on sim2real transfer of driving policies. They further give the opportunity of using reinforcement learning, instead of imitation learning, to acquire driving behaviours \cite{roach,endtoendRL}. Neural driving policies in recent years developed within such simulation environments can be categorised in two main families:

% One application domain that involves similar challenges to driving is offline motion trajectory forecasting \cite{rulesroad,multipath,multimodal,DESIRE,trevorcar,R2P2,precog,wayformer, scenetransformer, autobots, stackedtransf, endtoendraquel}. While evaluating driving performance requires a simulator, evaluating offline trajectory performance only requires a datasets of driving trajectories. There are multiple such datasets, such as, Argoverse \cite{Argoverse}, Waymo Open Dataset \cite{Sun_2020_CVPR}, and nuScenes \cite{nuscenes}, to name a few.
% \todo{BRIAN what are other datasets?}. 
%Imitation learning for offline trajectory prediction or closed-loop control suffers from multimodality of expert trajectories. Regressing car waypoints assumes that a car waypoint follows a unimodal Gaussian distribution in the 2D BEV space. 
%Building upon progress in generative models, motion trajectory decoders have been proposed that can model multimodal trajectory distributions.
% Many methods attempt to predict a distribution over future trajectories instead of a single trajectory, for the ego-vehicle or coordinated among multiple agents in the scene.  Tang and Salakhutdinov use conditional variational autoencoders (CVAEs) with discrete latent variables  \cite{multiplefutures}, Rhinehart \etal \cite{R2P2} use symmetric cross-entropy losses between predicted and ground-truth trajectory distributions,  Ngiam \etal \cite{scenetransformer} use multiple prediction heads with join classification and regression losses, Girgis \etal use set latent  variables \cite{autobots}. %, Zhong \etal use  diffusion models \cite{controllabletraffic}. 


Learning to drive from imitating  driving demonstrations is prevalent in the research and development of autonomous vehicles \cite{DBLP:journals/corr/abs-1710-02410,endtoendNVIDIA,gaildriving}.  %All methods 
Driving policies can take as input pixel and LiDAR input \cite{alvinn,endtoendNVIDIA,LBC,LAV,transfuser}, or use ground-truth perception of lanes, vehicles,  traffic signs and their  state attributes \cite{chauffernet,plant,roach}. In both cases, most methods predict  waypoints for the vehicle to follow, conditioned on a scene and a  distant goal representation. %Though learning from demonstrations is an established learning method, 
Most imitation learning methods optimize an objective that boils down to cloning the actions of the expert, as proposed  by Pomerleau decades ago \cite{alvinn}. Behaviour cloning has an underlying assumption of a unimodal Gaussian distribution for the actions to predict, which cannot handle  multimodality of  experts' driving behaviours, especially prevalent during accelerations, lane changes, merges, etc. . % Indeed, some many drive faster or slower, merge or bypass a car. %, and such multimodality cannot be adequately modelled by a unimodal Gaussian distribution.   
%hurts action regression, which is essentially what almost all methods have been using. 
%The limitations of behaviour cloning in the presence of multimodal action distributions is well documented in the literature \cite{}. 
Objectives and architectures that can better handle multimodal trajectory prediction have been  proposed,  
such as, mixture of expert  trajectory decoders \cite{wayformer}, combining classification and regression losses \cite{shafiullah2022behavior}, using Gaussian trajectory mixtures \cite{Kim_2023},   
conditional variational autoencoders (VAEs) with continuous or discrete latent variables \cite{multiplefutures, fragkiadaki2017motion}, producing heatmaps over a 2D bird's-eye-view  map to sample waypoint trajectories from \cite{lookout}. 

% such as, conditional VAEs with continuous or discete latent variables \cite{}, Gaussian mixture models \cite{}, or having multiple heads that are scored \cite{},  combination of regression and classification losses \cite{}.
 
%Most have been tried for offline traj. prediction and not for closed loop control. We compare with behaviour transformer in our experimental section.





%either drive from pixel and LiDAR input\cite{alvinn,endtoendNVIDIA,LBC,LAV,transfuser}, or use ground-truth perception of lanes, vehicles,  traffic signs and their  state attributes \cite{chauffernet,plant,roach}. The former set of methods build  neural architectures that lift 2D perspective camera features to stable 3D feature maps, or directly fuse perspective feature to predict  future waypoint trajectories; 
%their performance on the CARLA leaderboard \cite{CARLA}, a popular driving simulation environment, is impressive and the driving performance has been steadily increasing over the years. 
%This set of methods
%Driving from pixels compounds mistakes of perception and driving behaviour.  The latter set of methods isolate mistakes of perception and driving behaviour and are motivated by the large-scale annotation efforts of the self-driving vehicle industry to annotate oriented 3d boxes of vehicles,  bikers, pedestrians and traffic sings, as well as the use of high definition maps.  Surprisingly, few models have been developed for the latter case; though numerous methods exist for offline vehicle motion trajectory forecasting from oracle overhead rasterized maps or scene graphs \cite{wayformer, scenetransformer, autobots}, very few attempt to drive using this representation. %As a result, it is often hard to know how muc

% \paragraph{Guided Diffusion}
% Sampling from diffusion models can be guided from different conditioning signals other than the noisy estimate and the diffusion timestep \cite{Dhariwal2021DiffusionMB,Ho2022ClassifierFreeDG}. 
% %In the field of robotics, diffusion models find applications on planning \cite{janner2022planning,Ajay2022IsCG,Huang2023DiffusionbasedGO}, %scene re-arrangement \cite{Kapelyukh2022DALLEBotIW,Liu2022StructDiffusionOD}, 
% %controllable motion optimization \cite{Zhong2022GuidedCD,Jiang_2023_CVPR}, and imitation learning \cite{chi2023diffusion,reuss2023goal}. 


\paragraph{Few-shot  Prompting of LLMs for Instruction Following}
LLMs trained from Internet-scale text have shown impressive zero-shot reasoning capabilities for a variety of downstream language tasks when prompted appropriately, without any weight fine-tuning \cite{DBLP:journals/corr/abs-2201-11903,DBLP:journals/corr/abs-2107-13586,brown2020language}. LLMs have been used to map instructions to language subgoals \cite{DBLP:journals/corr/abs-2012-07277,DBLP:journals/corr/abs-1909-13072,huang2022language,https://doi.org/10.48550/arxiv.2207.05608} or python programs \cite{liang2022code,surís2023vipergpt,Gupta_2023_CVPR} with appropriate plan-like prompts. The predicted  programs or subgoals  interface with  low-level policies \cite{https://doi.org/10.48550/arxiv.2204.01691,singh2022progprompt,liang2022code} or pretrained vision-language detectors \cite{surís2023vipergpt,Gupta_2023_CVPR}. 
The scene description is usually provided in a symbolic form as a list of objects present, predicted by open-vocabulary detectors \cite{DBLP:journals/corr/abs-2104-12763}. 
Works of \cite{liang2022code,https://doi.org/10.48550/arxiv.2209.00465}  also feed as input overhead BEV spatial coordinates of objects to inform the LLM's predictions. 
Our work is most related to code-as-policies \cite{liang2022code} and extends it to the driving domain and language instructions there in. Instead of interfacing with ready low-level pick and place manipulation controllers as \cite{liang2022code}, we use the set of waypoints and corresponding cost maps predicted by the programs to  control a  diffusion-based driving policy. In that sense, we do not expect the LLM to know how to drive; this is the responsibility of the driving diffusion model. The LLM is merely responsible for interpreting language as cost maps to guide trajectory diffusion sampling. %For example, the instruction \textit{``merge in the left lane"} should predict a program that outputs low cost for all waypoints in the left lane; the one most suitable to reach based on the current velocity and scene context should be selected during guided trajectory diffusion sampling.



% Parallely, controlling an autonomous vehicle in natural language will  enable  human passengers to influence the vehicle's route and behaviour beyond supplying a final goal destination. Passengers would be able to give feedback to the vehicle and suggest places to park, intermediate stops, vehicles to follow, lanes to prefer or change, or speed to use. Language controllability of an autonomous vehicle is important for versatility and personalization of the vehicle-human experience,  and for reinforcing trust and transparency  in human-vehicle interaction. 

% Our language controllability builds upon code-as-policies \cite{liang2022code} in that it  prompts LLMs to predict programs for parsing instructions. Instead of predicting coordinate locations for pick and place control primitives which directly  parametrize the robot actions, our model combines predicted waypoints with a trajectory diffusion model to predict actions that both comply with a trajectory prior and attempt to follow the instruction. In that sense, we do not expect the LLM to know how to drive; this is the responsibility of the driving diffusion model. The LLM is merely responsible for interpreting language as cost maps to guide trajectory diffusion sampling. For example, the instruction \textit{``merge in the left lane"} should predict a program that outputs low cost for all waypoints in the left lane; the one most suitable to reach based on the current velocity and scene context should be selected during guided trajectory diffusion sampling.
%LLMs were used to generate task curricula and predict skills to execute in Minecraft worlds \cite{zhu2023ghost,lifshitz2023steve1}. Methods of \cite{wang2023voyager} use privileged information from the Minecraft simulator's interface regarding failures, state and inventory which they use to feedback to an LLM to plan and re-plan based on sub-goal successes and failures. LLMs are used as knowledge bases in place of traditional tuple based knowledge  \cite{roberts2020knowledge,brown2020language}. 


Close to our work are the recent method of \cite{controllabletraffic} and concurrent work of \cite{MotionDiffuser}. %While these methods 
%\todo{DETAILS:
They both show that diffusion models can be used for forecasting offline vehicle trajectories, and controlling  them via attracting them or repelling them from specific waypoints, or using cost maps related to traffic rules. % using classifier free guidance.} 
The methods are motivated by controllability of diffusion models at inference time. 
%Work of \cite{MotionDiffuser} further evaluates offline trajectory performance using minSADE, a top-6 trajectory matching metric, and shows state-of-the-art performance. 
%The proposed models do not outperform the previous work in offline trajectry prediction in the 
%None compares on estblished benchmarks  and not by improved offline trajectory performance. 
Our work is inspired by these works; instead of offline trajectory prediction it is the first to use diffusion policies for closed-loop driving and outperform previous formulations in nuPlan. %While in top-1 offline trajectory prediction error our method is worse than the baselines, it is able to better captures the trajectory distribution in rare  scenarios such as turns, leading in improved online driving performance. 
%Our experiments show that this is significant: the offline performance of diffusion policy was worse than existing deterministic alternatives. However, in rare scenarios critical for driving, diffusion better captures the trajectory distribution, leading in improved driving performance. 
Furthermore, we are the first to show language controllability of diffusion policies by marrying diffusion with LLM prompting for instruction-to-program generation. %\todo{++}



==> prompts/prompt.tex <==

\begin{figure}[ht]
  \centering
\begin{lstlisting}[language=Python, literate={-}{-}1]

# Python script for controlling a self-driving car
import numpy as np
from shapely.geometry import *
from shapely.affinity import *
from env_utils import get_ego_features, get_agent_features, get_lane_features

ego_features = get_ego_features()
agent_features = get_agent_features()
lane_features = get_lane_features()

# Drive to the closest car's current position
ego_pos = ego_features[:2]
agent_pos = agent_features[:,:2]
dists = np.linalg.norm(ego_pos[None] - agent_pos, axis=-1)
closest_agent_pos = agent_pos[dists.argmin()]
ret_val = closest_agent_pos

# Drive to the leftmost car
leftmost_car_idx = np.argmin(agent_pos[:,0])
leftmost_car_pos = agent_pos[leftmost_car_idx]
ret_val = leftmost_car_pos

# Drive behind the rightmost car
rightmost_car_idx = np.argmax(agent_pos[:,0])
rightmost_car_pos = agent_pos[rightmost_car_idx]
rightmost_car_heading = agent_features[rightmost_car_idx,2]
behind_offset = np.array([0,-1])
rot_matrix = np.array([[np.cos(rightmost_car_heading), -np.sin(rightmost_car_heading)],
[np.sin(rightmost_car_heading), np.cos(rightmost_car_heading)]])
behind_offset = rot_matrix @ behind_offset
destination_pos = rightmost_car_pos - behind_offset
ret_val = destination_pos

# Change to the leftmost lane that's in front of me
ego_pos = ego_features[:2]
ego_heading = ego_features[2]
ego_normal = np.array([np.cos(ego_heading), np.sin(ego_heading)])
lanes_in_front = []
for lane in lane_features:
    center = lane.mean(0)
    offset_to_ego = center - ego_pos
    if np.dot(ego_normal, offset_to_ego) > 0:
        lanes_in_front.append(lane)
sorted_lanes_in_front = sorted(lanes_in_front, key=lambda lane: np.min(lane[:,0]))
ret_val = sorted_lanes_in_front[0].mean(0)

# wait for pedestrians and cars to pass by, before changing lanes to the right

\end{lstlisting}
  \caption{Prompt for LLM}
  \label{fig:prompt}
\end{figure}

\begin{figure}[ht]
  \centering
\begin{lstlisting}[language=Python, literate={-}{-}1]

import time

# Check if cars are passing on the right
passing_cars_right = False
for agent in agent_features:
    if agent[0] > ego_pos[0]:
        passing_cars_right = True
        break

# Wait for cars to pass on the right
while passing_cars_right:
    # Get updated agent positions
    agent_features = get_agent_features()
    agent_pos = agent_features[:,:2]

    # Check if cars are still passing on the right
    passing_cars_right = False
    for agent in agent_features:
        if agent[0] > ego_pos[0]:
            passing_cars_right = True
            break

    # Wait for a short period of time before checking again
    time.sleep(0.1)

# Change to the rightmost lane
rightmost_lane = sorted_lanes_in_front[-1]
ret_val = rightmost_lane.mean(0)

\end{lstlisting}
  \caption{Output from LLM}
  \label{fig:output_llm}
\end{figure}


